Do the Hard Stuff First: Scheduling Dependent Computations in Data-Analytics Clusters

We present a scheduler that improves cluster utilization and job completion times by packing tasks having multi-resource requirements and inter-dependencies. While the problem is algorithmically very hard, we achieve near-optimality on the job DAGs that appear in production clusters at a large enterprise and in benchmarks such as TPC-DS. A key insight is that carefully handling the long-running tasks and those with tough-to-pack resource needs will produce good-enough schedules. However, which subset of tasks to treat carefully is not clear (and intractable to discover). Hence, we offer a search procedure that evaluates various possibilities and outputs a preferred schedule order over tasks. An online component enforces the schedule orders desired by the various jobs running on the cluster. In addition, it packs tasks, overbooks the fungible resources and guarantees bounded unfairness for a variety of desirable fairness schemes. Relative to the state-of-the art schedulers, we speed up 50% of the jobs by over 30% each.

==> texfiles/background.tex <==
%!TEX root=../graphene.tex
\section{Analyzing DAGs in Production}
\label{sec:background}
\label{subsec:DAG-analysis}
\label{subsec:potential-gains}
To ground the discussion, we examine the production jobs from 
a cluster of tens of thousands of servers at Microsoft that runs
jobs written in the SCOPE~\cite{SCOPE} language. We also analyzed
jobs from several other clusters that ran Hive/Hadoop jobs and
HPC workload~\cite{condor}.
\cut{
Microsoft's cluster consisting tens of thousands of servers. Users
write jobs in a high level language~\cite{SCOPE} which is then
compiled to a directed acyclic graph (DAG) by a query optimizer. 
We
also analyzed the jobs from several internal clusters that ran
Hive/Hadoop jobs as well as a high-performance computing~(HPC)
workloads~\cite{condor}.}

We analyzed DAGs along the following dimensions:
\begin{Itemize}
\item {\bf How deep are the DAGs?} By depth,
  we refer to the number of tasks on the critical path. A map-reduce
  job has depth $2$. Intuitively, the deeper a DAG, the more
  carefully one has to consider dependencies. We find that the median
  (75th, 95th percentile) DAG has depth 7 (10, 17).

\item {\bf How diverse are the resource demands?}  Table~\ref{tab:resource_cov}
shows the coefficient-of-variation~(CoV) across tasks for various resources.
% across different clusters.
We find that resource demands vary substantially. 
HPC clusters appear to have less variability than data-parallel clusters.
The variability is possibly due to differences in work at
  each task---some are compute heavy~(e.g., user-defined code for
  video rendering) whereas others are memory heavy~(e.g., in-memory sorts).
%  and still others are network heavy~(e.g., shuffles). 

\item{\bf Where does the work lie?}
Let ${\tt CPMass}$ be the total work in the stages on the critical path.
From Table~\ref{tab:whereIsMass}, $42$\% of DAGs have ${\tt CPMass}$ above $80$\%.
Critical path aware schedulers do well for such DAGs.% since one chain dominates.
Let ${\tt UnconstrainedMass}$ be the total work in stages with no parents (i.e., no dependencies).
We see that roughly $33$\% of the DAGs have ${\tt UnconstrainedMass}$ above $80$\%. 
Such DAGs will benefit from packing schedulers.
The above cases are not mutually exclusive and together account for $54$\% of DAGs. 
For the other $46$\% of DAGs, neither packers nor criticality-based schedulers may work well. 
\end{Itemize}

\begin{table}[t!]
\centering
{\scriptsize
\begin{tabular}{p{.58in}||c|c|c|c|c|c|c}
& {CPU} & {Mem.} & \multicolumn{2}{c|}{Network} & \multicolumn{2}{c|}{Disk} \\\cline{4-7}
& & & Read & Write & Read & Write\\\hline
Bing DAGs & 0.76 & 1.01 & 1.69 & 7.08 & 1.39 & 1.94 \\\hline
Hive/ Hadoop & 0.89 & 0.42 & 0.77 & 1.34 & 1.59 & 1.41  \\\hline
HPC~(Condor) & 0.53 & 0.80 & N/A & N/A & \multicolumn{2}{c|}{1.55 (R+W)} \\
\end{tabular}
}
\caption{Coefficient-of-variation~($={\mbox{stdev.}}/{\mbox{avg.}}$) of tasks' demands for various resource. Across three examined frameworks, tasks exhibit substantial variability~(CoV $\sim 1$) for many resources.\label{tab:resource_cov}}
\end{table}
\begin{table}[t!]
\centering
{\scriptsize
\begin{tabular}{p{.6in}|c|c|c|c|c}
\multirow{2}{*}{"Mass" that is \ldots}& \multicolumn{5}{c}{Percentage of total work in the DAG}\\
& [0-20) & [20-40) & [40-60) & [60-80) & [80-100]\\\hline
{on CriticalPath} & 14.6\% & 13.2\% & 15.2\% & 15.3\% & {\bf 41.6}\%\\%\hline
{"unconstrained"} & 15.6\% & 20.4\% & 14.2\% & 16.4\% & {\bf 33.3}\%\\%\hline
{"unordered"} & 0 & 3.6\% & 11.8\% & 27.9\% & {\bf 56.6}\% \\\hline
\end{tabular}
}\caption{Histogram of where the work in a DAG lies. For e.g., in $14.6\%$ of DAGs, 
the mass on their critical path is $\in [0, 20)\%$ of the total work in that DAG.\label{tab:whereIsMass}}
\end{table}
\begin{figure}[t!]
\includegraphics[width=2in]{figures/gap.pdf}
\caption{CDF of \emph{gap} between DAG runtime and several lower bounds. 
Gap is computed as $100\cdot\frac{runtime-lowerbound}{runtime}$. \label{fig:gap}}
\end{figure}

To quantify the potential gains, we compare the runtime of the DAGs in production 
to some measures. Our first measure, ${\tt CPLength}$ is the duration of the DAG's critical path. 
A DAG would take no longer if the available parallelism is infinite.
The second measure, ${\tt TotalWork}$, is 
the total work in the DAG normalized by the cluster share of that DAG. 
If there were no dependencies and perfect packing, a DAG would take no longer.
In practice, DAGs do take longer than these measures.
We define \emph{gap} as ${\small\sf 1- \frac{\mbox{measure}}{\mbox{duration}}}$. 
A gap of 50\% implies twice the execution time of the baseline. 
Fig.~\ref{fig:gap} plots a CDF over all DAGs. 

Observe that half of the jobs have a gap of over $70$\% for both these estimates.
That is, half the jobs take over $4\times$ longer than they should.
%Some DAGs are closer to their CPLength metric, others to their TotalWork metric. 
Both of the above measures however are loose. The first ignores all the
work off the critical path and the second ignores dependencies. The
gap over an improved lower bound~(see~\xref{sec:betterlb}) is
smaller: half of the jobs are off by $2\times$.  

A few
complications are worth noting for this result. First, some DAGs
finish faster than their ${\tt TotalWork}$ estimate because our production
scheduler is work conserving and can give jobs more than their fair
share. Second, we discount the effects of  stragglers and 
failures~\cite{mantri} on job runtimes in two ways: (1) Use
the fastest execution over groups of related jobs~(e.g., recurring jobs
in~\cite{rope}) and (2) deduct the duration wherein the job has $<10$
tasks executing.  We conclude that the runtimes in production 
exhibit substantial room for improvement.

Let ${\tt MaxUnorderedMass}$ be the work in the largest set of stages 
that are neither parents nor children of each other. Table~\ref{tab:whereIsMass} shows that 
$57$\% of DAGs have ${\tt MaxUnorderedMass}$ above $80$\%. That is, if ancestors of the 
unordered stages were scheduled appropriately, substantial gains can accrue from packing tasks in the maximal 
unordered subset.

From the above analysis, we observe that (1) production jobs have
large DAGs that are neither a bunch of unrelated stages nor a chain of stages, 
and (2) a packing+dependency-aware scheduler can offer substantial improvements.

==> texfiles/d.tex <==
%!TEX root=../paper.tex

\section{\namesec Scheduler}
\label{sec:design}

In this section, we describe {\name}'s scheduling heuristic, assuming complete knowledge of the resource requirements of tasks and resource availabilities at machines; we explain how to estimate these in~\xref{sec:system}. We begin with an analytical model that explains the computational complexity of our problem~(\xref{subsec:model}). We then develop heuristics that match tasks to machines so as to reduce makespan (\xref{subsec:packing}) and average job completion time (\xref{subsec:completion}). Finally, we combine these heuristics with a large class of fairness algorithms~(\xref{subsec:fairness}).

%We begin by constructing an analytical model that allows us to
%evaluate the complexity of our scheduling problem when resource
%estimates of tasks are exposed to the scheduler during allocation.
%Our analysis shows that when factoring multiple resources in the
%allocation step the scheduling problem is APX-hard
%(Section~\ref{subsec:model}).  We then develop heuristics to
%\emph{pack} tasks on machines thereby improving cluster/job throughput
%(Section~\ref{subsec:matching}).

\subsection{Analytical model}
\label{subsec:model}
\camera{
To connect the task scheduling problem with prior theoretical work, we cast it into a general optimization framework.} 
%We first specify the notations for resource demands and matching variables, before using them to define the constraints and the objective function.

\vskip .05in
\noindent{\bf Notations:} We consider demands of tasks along four resources: CPU, memory, disk, and network bandwidth~(see Table~\ref{tab:task_resource_demands}). For every resource $r$, we denote ($i$) the capacity of that resource on machine $i$ as $c_i^r$, and ($ii$) the demand of task $j$ on resource $r$ as $d_j^r$.

\begin{table}[t!]
\begin{small}
\begin{tabular}{p{.6in}|p{2.4in}}
{\bf Term} & {\bf Explanation}\\\hline
$d_j^{\text{cpu}}, f_j^{\text{cpu}}$ & CPU demand (i.e., cores)~($d$) and cpu cycles~($f$) \\[.05in]\hline
$d_j^{\text{mem}}$ & Peak memory used by task \\[.05in]\hline
$d_j^{\text{diskR}}, d_j^{\text{diskW}}$, $f_{ij}^{\text{diskR}}, f_{j}^{\text{diskW}}$ & Peak disk read/write bandwidth of the task~($d$), bytes to be read from machine $i$ and output~($f$)  \\[.05in]\hline
$d_j^{\text{netIn}}, d_j^{\text{netOut}}$ & Peak network bandwidth in/out of a machine that the task can use~($d$)\\ \hline\hline
\end{tabular}
\end{small}
\caption{Resource demands of task $j$. Note that the demands for network resource depend on task placement.
}
%bytes to be moved over the network depend on task placement (and so also the demand for network bandwidth).}
\label{tab:task_resource_demands}
\end{table}

Next, we define variables that encode the task schedule and resource allocation. Note that allocation happens across machines (spatial) and over time (temporal). Let $Y_{ij}^t$ be an indicator variable that is $1$ if task $j$ is allocated to machine $i$ at time $t$ (time is discretized). Also, task $j$ is allocated $X_{ij}^{r,t}$ units of resource type $r$ on machine $i$, at time $t$. \camera{Let $i^*_j$ denote the machine that task $j$ is scheduled at and $\text{start}_j$ and $\text{duration}_j$ denote the corresponding aspects of task $j$.\footnote{Though we use $\text{start}_j$ and $i_j^*$ in the constraints below for convenience, note that they are unknown apriori. Hence, all their occurrences need to be replaced with equivalent terms using the indicator variables $Y_{ij}^t$. For example $X_{i_j^*j}^{r,t} = \sum_i Y_{ij}^t X_{ij}^{r,t}.$}} We do not model preemption here for simplicity. Note that a task may need network and other resources at multiple machines in the cluster due to remote reads.

\vskip .05in
\noindent{\bf Constraints:} 
%Our main constraints during such an allocation are to not over-allocate resources on a machine or to a task. % Thus, 
\camera{First}, the cumulative resource usage on a machine $i$ at any given time cannot exceed its capacity:
\begin{equation}
\sum_j X_{ij}^{r,t} \leq c_i^r, \forall{i, t, r}.
\label{eqn:alloc_cap}
\end{equation}
Second, tasks need no more than their peak requirements and no resources are allocated when tasks are inactive.
\begin{eqnarray}
0 \leq X_{ij}^{r,t} \leq d_j^r, \forall{r, i, j,t}.\label{eqn:alloc_peak}\\
\forall_{i, r, t}\  X_{ij}^{r,t} = 0 \mbox{ if } t \notin [\text{start}_j, \text{start}_j+\text{duration}_j].
\end{eqnarray}
Third,  to avoid costs of preemption, schedulers may prefer to uninterruptedly allot resources until the task completes.
\begin{equation}
\sum_{t=\text{start}_j}^{\text{start}_j  + \text{duration}_j} Y_{ij}^t = 
\left\{
\begin{array}{ll}
\text{duration}_j & \mbox{machine $i = i_j^*$}\\
0 & \mbox{other machines}
\end{array}\right.
\label{eqn:indicator_runtime}
\end{equation}
Fourth, the duration of a task depends on task placement and resource allocation:
\begin{equation}
\text{duration}_j = \max \left(
\begin{array}{l}
\frac{f_j^{\text{cpu}}}{\sum_{t} X_{i_j^*j}^{\text{cpu},t}}, 
%\frac{d_j^{\text{mem}}}{\sum_{t} X_{i^*j}^{\text{mem},t}}\\
\frac{f_j^{\text{diskW}}}{\sum_{t} X_{i_j^*j}^{\text{diskW},t}}, \\
\forall i \ \ \frac{f_{ij}^{diskR}}{\sum_{t} X_{ij}^{\text{diskR},t}}, \\
\frac{\sum_{i\neq i_j^*}f_{ij}^{diskR}}{\sum_{t} X_{i_j^*j}^{\text{netIn},t}},\\
\forall i \neq i_j^*, \ \  \frac{f_{ij}^{diskR}}{\sum_{t} X_{ij}^{\text{netOut},t}}\\
%\frac{f_{ij}^{diskW}}{\sum_{t} X_{ij}^{\text{netOut},t}}
\end{array}
\right)
\label{eqn:runtime}
\end{equation}
In each term, the numerator(f) is the total resource requirement (e.g., cpu cycles or bytes), while the denominator is the allocated resource rate (e.g., cores or bandwidth). 
From top to bottom, the terms correspond to cpu cycles, writing output to local-disk, reading from (multiple) disks containing the input, network bandwidth into the machine that runs the task and network bandwidth out of other machines that have task input.
%\footnote{$d_{ij}^{in}$ is the amount of task $j$'s input that is present on node $i$ and $d_j^{out}$ is the size of its output.} 
Note here that cores and memory are only allocated at the machine that the task is placed at but the disk and network bandwidths are needed at every machine that contains task input. We assumed here for simplicity that task output just goes to local disk and that the bandwidths are provisioned at each time so as to not bottleneck transfers, i.e., $$\forall{t, j, i \neq i_j^*}\ \ X_{ij}^{\text{netOut}, t} \geq X_{ij}^{\text{diskR},t} \text{ and } X_{i_j^*j}^{\text{netIn}, t} \geq \sum_{i\neq i^*}X_{ij}^{netOut,t}.$$ We also assumed that the task is allocated its peak memory size since unlike the above resources, tasks' runtime can be arbitrarily worse (due to thrashing) if it were allocated less than its peak required, i.e., $  \forall t \ \ X_{i_j^*j}^{\text{mem},t} = d_j^{\text{mem}}$.

\begin{table}[t!]
\begin{small}
\begin{tabular}{p{.6in}|p{2.4in}}
{\bf Term} & {\bf Explanation}\\\hline
$c_i^{\text{cpu}}, c_i^{\text{mem}}$ & Number of cores, Memory size\\
$c_i^{\text{diskR}}, c_i^{\text{diskW}}$ & Disk read and write bandwidth\\
$c_i^{\text{netIn}}, c_i^{\text{netOut}}$ & Network bandwidth in/out of machine\\
\end{tabular}
\end{small}
\caption{Resources measured at machine $i$. Note that the availability of these resources changes as tasks are scheduled on the machine.\label{tab:machine_rsrc}}
\end{table}
\vskip .05in
\noindent{\bf Objective function:} 
\camera{
Our setup lends itself to various objective functions of interest to distributed clusters including minimizing {\em makespan}~\footnote{Makespan = $\max_{\mbox{job}\ J} \max_{\mbox{task}\ j \in J} \max_{\mbox{time}\ t} (Y_{ij}^t>0)$} and {\em job completion time}~\footnote{Job $J$'s finish time is $\max_{\mbox{task } j \in \mbox{ job } J} \max_{\mbox{time }t} (Y_{ij}^t >0)$}. Minimizing makespan is equivalent to maximizing packing efficiency. 
%Job completion time is the duration between its arrival and the end of its last task. 
Further, we can pose fairness as an additional constraint to be meet at all times.\footnote{Dominant resource share of $J$ at time $t$ $=\max_{\mbox{resource }r} \frac{\sum_{i, j\in J} X_{ij}^{r,t}}{\sum_i c_i^r}$.} % Small jobs, that execute all their tasks in parallel, have a duration equal to the maximum of their task durations. \footnote{An alternate metric is to minimize cluster occupancy: $\sum_{i,j,t} Y_{ij}^t$. Our work, however, focuses on the user centric metric of job duration.}
}


\vskip .05in
\noindent{\bf Takeaways: }
\camera{
The above analytical formulation is essentially a hardness result.
Regardless of the objective, several of the constraints are non-linear.
Resource malleability~(eqn:\ref{eqn:alloc_peak}), task placement~(eqn:\ref{eqn:runtime}) and how task duration relates to the resources allocated at multiple machines~(eqn:\ref{eqn:runtime}) are some of the complicating factors. Fast solvers are only known for a few special cases with non-linear constraints~(e.g., the quadratic assignment problem).
Finding the optimal allocation, therefore, is computationally expensive.
Note that these non-linearities remain {\em inspite} of
ignoring the dependencies between tasks~(e.g., the DAG) and the several simplifications used throughout (e.g.,  no task preemption). 
In fact, scheduling theory shows that even when placement considerations are eliminated, the problem of packing multi-dimensional balls to minimal number of bins is APX-Hard~\cite{apx}. 
Worse, re-solving the problem whenever new jobs arrive requires online scheduling.
For the online case, recent work also shows that no polynomial time approximation scheme is possible with competitive ratio of the number of dimensions unless NP=ZPP~\cite{tightVectorPacking}.}


\camera{
Given this computational complexity, unsurprisingly, cluster schedulers deployed in practice do not attempt to pack tasks. All known research proposals rely on heuristics.  We discuss them in further detail later, but note here that we are unaware of any that considers multiple resources and simultaneously considers improving makespan, average job completion time and fairness considerations. Next, we develop heuristics for packing efficiency~(\xref{subsec:packing}), job completion time~(\xref{subsec:completion}) and incorporate fairness~(\xref{subsec:fairness}).
}

\subsection{Packing Efficiency for Makespan}
\label{subsec:packing}

% multi-dimensional bin packing, 1D solution
\camera{
Packing tasks to machines is analogous to the multi-dimensional bin packing referred above. To develop an efficient heuristic, we draw an analogy with the solution in a one-dimensional space (both balls and bins). An effective heuristic proceeds by repeatedly matching the largest ball that fits in the current bin; when no more balls fit, a new bin is opened.  Intuitively, this approach reduces the unused space in each bin (i.e., reduces fragmentation) and therefore, reduces the total number of bins used.  In one-dimensional space, this heuristic requires no more than $(\frac{11}{9})$OPT+$1$ bins, where OPT is the optimal number of bins~\cite{vazirani}.}

\vskip .05in
\noindent{\bf Alignment:}
We extend the above heuristic by defining {\em alignment} of a task relative to a machine across multiple dimensions. Similar to the one-dimensional case, the larger the alignment the lower the fragmentation. We considered many options for defining the alignment. Among them, the best packing efficiency was obtained using the dot product between task requirements and resource availabilities on machines. 

Our allocation operates as follows. When resources on a machine become available, the scheduler first selects the set of tasks whose peak usage of each resource can be accommodated on that machine. For each task in this set, \name computes an {\it alignment score} to the machine. The alignment score is a weighted dot product between the vector of machine's available resources and the task's peak usage of resources. The task with the {\em highest} alignment score is scheduled and allocated its peak resource demands. This process is repeated recursively until the machine cannot accommodate any further tasks. 

\camera{
Picking tasks as above has these properties. First, only tasks' whose peak demands are satisfiable are considered; so over-allocation is impossible. Under-utilization of resources is possible, however, we discuss how to mitigate that using a resource tracker in~\xref{subsec:learn}. Second, the alignment score is largest for the task that uses the most resources on the machine along every resource type. Third, if a particular resource is abundant on a machine, then tasks that require that resource will have higher scores compared to tasks that use the same amount of resources overall. Together, this reduces fragmentation; loosely, bigger balls are placed first and machine resources that are currently abundant are used up before those that are currently scarce by choosing tasks appropriately.}

\camera{
When computing the dot product, {\name} normalizes the task requirements as well as available resources on the machine by the machine's overall capacity. This ensures that the numerical range of a machine's resource (e.g., 16 cores vs. 96GB of RAM) and tasks' demands (e.g., 4 cores vs. 1 Gbps network) do not affect the alignment score. All the resources are weighed equally.
}

% IO
\vskip .05in
\noindent{\bf Incorporating task placement:} 
\camera{
A subtle aspect in calculating the alignment score is to appropriately adjust the disk and network demands based on task placement. Recall that while CPU and memory allotment are primarily local, disk and network resources may be needed at multiple machines if data is read (or written) remotely. 
For remote reads, {\name} checks before placing a task on a machine that sufficient disk read and network-out bandwidth are available at each of the remote machines that contain task input and that sufficient network-in bandwidth is available at the local machine. Including these remote resources in the alignment score computation~(dot product) is problematic. The vectors become as large as the number of machines in the cluster. Also, since the score is higher for tasks that use more resources overall, remote placement is preferred! Instead, {\name} computes  the alignment score with only the local resources and imposes a remote penalty (of, say, $10\%$) to penalize use of remote resources. We run sensitivity analysis on the value of this remote penalty in~\xref{subsec:e_sensitivity}. Together, this ensures that over-allocation is still impossible, fragmentation is reduced and using local resources is preferred. Consequently, the network and remote disks are free for tasks that compulsively need them. 
}
\subsection{Average Completion Time}
\label{subsec:completion}

Achieving packing efficiency does not necessarily improve job completion time. \camera{Consider two jobs running on a two machine cluster. Machines have $2$ cores and $4$GB of memory. The first job has six tasks each requiring $\langle2\ \text{cores}, 3\ \text{GB}\rangle$ while the second job has two tasks requiring $\langle1\ \text{cores}, 2\ \text{GB}\rangle$. Tasks of the first job have higher alignment score. Hence, the above packing efficiency heuristic schedules all tasks of the first job before the second job's tasks. Assuming all the tasks have the same duration, it is easy to see that swapping the order lowers average job completion time.}

\camera{
A useful starting point to reduce average job completion time is the shortest-remaining-time-first (SRTF) algorithm~\cite{mor}. SRTF schedules jobs in ascending order of their remaining time. While one can extend SRTF to consider multiple resource requirements of tasks, its greedy scheduling approach nonetheless leads to resource fragmentation~\cite{vector}. The consequent loss in packing efficiency delays the scheduling of other waiting jobs, thus inflating their durations. Therefore, the challenge in improving job completion time is to {\em balance prioritization of jobs that have less remaining work against loss in packing efficiency}.}

 % SRTF is greedy and schedulers use SRTF by considering the number of tasks as a proxy for job duration. While the number of tasks is a reasonable approximation when task durations are a function of only one resource, extending it across multiple resources is tricky. When tasks consume multiple resources, we need to holistically consider all of them. Further, even when all resources are considered, the chances of their fragmentation with greedy approaches like SRTF increases with the number of dimensions. The ensuing loss in packing efficiency may in turn adversely inflate job durations. Resolving this tension is key to optimizing completion time in multi-resource schedulers. 

%We first develop a heuristic to prioritize jobs with the least remaining work in a multi-resource setting and then combine it with our packing efficiency heuristic from \xref{subsec:packing}.

\subsubsection{Shortest Remaining Time}
\label{subsubsec:small}

% objective, problems: accounting for multiple resources
We first extend the SRTF scheduling algorithm to incorporate multiple resources. Consider scheduling jobs in increasing order of their number of remaining tasks. The fewer tasks remaining in a job, the lower is its remaining duration. However, tasks can have different durations. Worse, tasks can have varying requirements for different resources. Scheduling a job with high resource requirements, even if it has the smallest duration, incurs the opportunity cost of not scheduling other jobs simultaneously. \camera{Intuitively, favoring jobs that have the least remaining work improves average completion time the most with the least effort.}

% remaining job duration, use history of tasks
\vskip .05in
\noindent{\bf Scoring job's remaining work:} 
\camera{
We calculate the total resource requirements of all remaining tasks of the job across all dimensions. 
To be immune to variations in numerical ranges of the different resources, we normalize the various resources as before.
The resource consumption of a task is the sum across all the (normalized) resource dimensions multiplied by the task duration. We estimate task duration based on earlier runs of the same or similar jobs as well as the completed tasks of the same phase. 
The score for a job is the total resource consumption of its remaining tasks.
}

% multiply
\camera{
Scheduling jobs with lower scores first reduces average completion time the most. The score prefers jobs with low duration mimicing the SRTF heuristic.  In addition, favoring jobs that need less resources has smaller opportunity cost since more resources are available for other jobs. 
}

\subsubsection{Combining with Packing Efficiency}
\label{subsubsec:algo}

% combine
Recall that we need to combine the above score with the packing efficiency heuristic since using only the above score can fragment resources which delays jobs and inflates cluster makespan.


% options: /, rank ordering; objective is equal representation
We combine the two metrics
---remaining resource usage and alignment score---using a weighted sum. Denoting the alignment score by $a$ and the remaining resource usage as $p$, we pick the task with the highest value of  $\left(a + \varepsilon\cdot p\right)$. To ensure that the expression is not dominated by 
\camera{either, we recommend $\varepsilon=\left(\bar{a} / \bar{p}\right)$, where $\bar{a}$ and $\bar{p}$ denote the average scores for alignment and remaining work. Note that $a$ is per-task, whereas $p$ is per-job. While the best choice of $\varepsilon$ depends on the workload, our evaluation shows that the gains from packing efficiency are only moderately sensitive to $\varepsilon$ since most jobs have pending tasks with similar resource profiles. Improving average job completion time, however, requires non-zero values of $\varepsilon$ though the gains stabilize quickly.
We will show in \xref{subsec:sim} that the above combination significantly improves over alternatives.
}


\subsection{Incorporating fairness}
\label{subsec:fairness}
As described so far, {\name} matches tasks to machines to improve cluster efficiency and job completion time without considering fairness. Fairness is a useful tool in shared clusters. Conversations with cluster operators indicate that proportional allocations improve performance predictability. However, it is not an absolute requirement and deviations in fairness for better performance are acceptable. 
Other properties such as strategy-proofness, envy freedom and sharing incentive are less important in private clusters since the organization can mandate sharing and audit jobs post facto. Here, we describe how {\name} balances performance with fair allocations. 

A common property to many fairness based schedulers is to keep track of the allocations of running jobs and offer the next available resource to the job that is farthest from its fair share. Slot based fairness~\cite{capacity, fair} has this property: the next slot is allocated to the job that occupies the fewest slots relative to its fair share. Likewise, DRF~\cite{drf} offers resources to the job whose dominant resource's allocation is furthest from its fair share.
\camera{ 
Similar to DRR scheduling, long-running or resource-hungry tasks~(alt: large packets) cause short-term unfairness during such allocation.
However, bounded task sizes (as in our clusters) limits the unfairness and, in practice, the above method offers fairness at meaningful timescales.}

\camera{
{\name} uses a {\em fairness knob} to trade-off fairness for performance. The knob $f$ takes values in the range of $[0, 1)$ and intuitively quantifies the extent to which {\name} adheres to fair allocations. When resources become available, {\name} sorts the jobs (set $J$) in decreasing order of how far they are from their fair share. Note that most fair schedulers already maintain such a list. It then looks for the best task (as before) among the runnable tasks belonging to the first $\lceil\left(1- f\right)\ J\rceil$ jobs in the sorted list. Setting $f=0$ results in the most efficient scheduling choice, whereas $f \rightarrow 1$ yields perfect fairness. In this way, {\name} can incorporate most policies for fairness.
}

\camera{
The trade-off between fairness and performance is rarely smooth. However, in 
scheduling tasks in data-parallel clusters, we find that the above knob lets {\name} achieve schedules that are both reasonably fair and reasonably efficient. For knob values in the range [0.25,0.5], {\name}'s makespan is within 10\% of the most-efficient (and most-unfair) schedule while delaying jobs by no more than 10\% compared to the fair schedulers. This is because though the fairness constraint restricts which jobs (or queues) the available resources can be offered to, there are many tasks pending in a job or queue and from among these many choices it is still possible to pick a task that aligns well with the resources on the machine to be allocated, leading to nearly the same packing efficiency.}


\subsection{Discussion}
\label{subsec:discuss}

\noindent{\bf DAG Awareness:} 
\camera{The last few tasks before a barrier~(e.g., sometimes, no reduce task can start before all maps finish) present a low-cost high-gain opportunity.  For the purpose of this discussion, the end of a job can also be considered a barrier. Delay in scheduling these tasks directly impacts job completion time. 
However, scheduling just these last few tasks preferentially has little impact on other jobs since it is taking away only a small amount of resources.  {\name} uses knowledge of the job's DAG to preferentially schedule the last few tasks before a barrier.  Given a barrier knob value $b \in [0, 1)$, whenever resources are available {\name} preferentially offers them to tasks that remain after $b$ fraction of tasks in the stage preceding a barrier have finished. Among these tasks, {\name} still ensures that sufficient resources are available and chooses based on alignment score.  Results in~\xref{subsec:e_sensitivity} show that values of $b\in [.85, .95]$ improve both job completion time and makespan.}

\vskip .05in
\noindent{\bf Starvation Prevention:} Initially, we were concerned that the above solution can {\it starve} tasks that have large resource demands. Since the scheduler assigns resources on a machine as soon as they are available, it could take a long time to accommodate large tasks. \camera{Note that DAG awareness kicks in only for the last few tasks of a job, and hence may not help. However, in practice, we do not encounter such starvation due to two reasons. First, recall from Figure~\ref{fig:profiles} that most tasks have demands within one order of magnitude of one another. As a result, it is likely that the machine resources that become free when one or a small number of tasks finish suffice to fit even the larger tasks. Second, machines report resource availability to the scheduler periodically (\xref{subsec:arch}). The intended goal was to keep the scheduler load low. But, doing so also causes the scheduler to learn about all the resources freed up by the tasks that finish in the preceding period together. A more principled solution that reserves machine resources for {\it starved} tasks is left to future work.}

\vskip .05in
\noindent{\bf Future Demands:} \camera{While our solution is online, we point out that (imperfect) knowledge of the future is already available.} Since each job manager knows its DAG, it knows the future tasks. The scheduler can also estimate when future machine resources become available; each job manager can estimate when an assigned task will finish similar to how they estimate tasks' resource demands. Using such future knowledge, the scheduler can better mimic the offline solution. We leave to future work how to extend the scheduler to use such future knowledge.

==> texfiles/design.tex <==
%!TEX root=../paper.tex
\section{{\namesec} Design}	
\label{sec:design}

argue that this is a new problem in the context of bigdata clusters (nature of the DAGs: stage with tasks); many simultaneously running DAGs in a cluster; placement constraints.

argue that this is a real and significant problem (impact on DAGs; at least the bigger DAGs with unconstrained runtimes)

argue that the new solutions work and are manageable

set up the architecture: {\name} works on the sidelines.  Given a collection of DAGs that remain and a desired cluster allocation, {\name} computes a good schedule. The schedule is communicated to the AMs and the RM which are guided by it in some fashion. Judicious over-allocation happens on the dynamic path.

-----------

levels make sense when all tasks are of same size; UET model in earlier work; they do not make sense when tasks have different durations

pipelining: ie overlapping several short duration tasks with a longer duration task is a source of wins

------------

\subsection{Gv1: Bottom-up clustering of tasks}
\label{subsec:gv1}
At a high level, this approach partitions the DAG into subsets such that 
(a) tasks in a subset have no dependencies
among themselves and (b) there exists a total order across subsets,
i.e., the subsets can be ranked numerically such that for every
dependency, the parent task is in subset with lower rank than the
child.  An example is shown in Figure~\ref{fig:p_eg3}, where the
colored underlays represent the different subsets. Subsets are chosen carefully to enhance packability of tasks within each subset~(\xref{subsec:gv1_group}).
Next, we schedule the subsets in level order. With modifications that account for placement preferences and dynamic promotions~(\xref{subsec:gv1_sched}).

Level scheduling has nice connections with widely-used algorithms; however the above version has a few novel aspects. Graph drawing tools~(e.g., GraphViz~\cite{XXX} and Microsoft AGL~\cite{XXX}) break a DAG into levels to enhance visiblity. So also do the early work on multi-processor scheduling; most notably the Graham-Coffman algorithm (G-C from now on)~\cite{XXX}. Even critical path scheduling can be thought of as a level scheduler~\footnote{Tasks' critical path length determines the level and the subset at each level consists of tasks having the same critical path length.}. We defer detailed comparisons to later~\xref{sec:related}, however none of the prior incarnations pick task subsets so as to enhance resource packability. Several do not consider placement constraints or allow for dynamic changes.

\subsubsection{Grouping into levels}
\label{subsec:gv1_group}
Initialize: put each task into a subset by itself; i.e., all subsets are of size 1.

Recursively:
First, 
find a pair of task subsets which when scheduled together finish faster than they would if scheduled separately and which do not inflate the critical path length.  Implicitly, this means that all of the tasks in the pair of subsets are {\em unordered}, i.e., have no dependency among themselves.  Further, the subset pair that offers the greatest reduction in runtime when scheduled together is the one whose resource demands pack the best.  

Second, 
collapse the pair into a single task subset.

Repeat.

The above process terminates when none of the subsets can be merged without inflating the critical path of the DAG.  

Finally, order these subsets such that for every dependency in the DAG, the subset containing the parent task receives a lower {\em index} than that containing the child.



\subsubsection{Efficient clustering}
We show how to do the clustering quite efficiently: (a) the duration to run both subsets together can be estimated by emulating a scheduling algorithm (b) the CP length post merger can be estimated by iteratively maintaining the longest path from the root and the leaf for each subset; for e.g., post merge the longest path from any root is the max of the longest path from root of the individual subsets (c) similarly iteratively maintain unordered relationships between subsets; the set of tasks that are unordered wrt task $t$, $U(t)$, is all tasks except the ancestors or descendants of task $t$. When merging subsets $s_1$ and $s_2$, the unordered tasks for the resultant subset $s$ is computed as $U(s) = U(s_1) \cap U(s_2)$. (d) cache the scores of subsets so as to speed up searching for pairs. (e) ordering subsets can be done by assigning some random order and swapping whenever a subset pair has the wrong order. 
{\bf edit: what is the complexity?}


\subsubsection{Dynamic scheduling of the ordered levels}
\label{subsec:gv1_sched}
We iteratively pick an unscheduled task from the smallest level. Break ties by considering placement, i.e., prefer to place tasks on machines where their resource use is small (e.g., data local placements).

If none of the tasks in the smallest level can use a machine, perhaps because available resources are smaller than task demands, we have two options. One, let these resources go idle. Two, pick a task from a higher level that can make use of these resources. We tried both approaches. In the latter, we pick among the tasks that can use the available resources, the one with the smallest level. We find this to work better in practice often but not always. The gains come from not letting resources go unused. The losses come when such dynamic promotions further delay when the task(s) in the smallest level can begin execution. When these tasks have many dependents downstream, doing so can inflate the critical path.  We found that a superior approach is to explicitly distinguish between these two cases. By looking at the expected completion times of other tasks, we anticipate when these passed-over tasks in the smallest level may be schedulable, i.e., when enough resources at a suitable machine will become free, and allow only those promotions that do not delay the completion time of the passed-over tasks so much as to impact the critical path. Implicitly, this ensures that tasks with a lot of dependents or dependents that are to be scheduled soon after this task finishes are not delayed by promotions of other tasks.

{\bf edit some of this probably requires more than ``ordered levels''; may need clusterstate}

\subsubsection{Findings}
This bottom-up approach works quite well on small DAGs. For e.g., it does the right thing on all the examples described in the paper thus far. However, we find that on larger DAGs from production jobs, the gains are not substantial.  The main reason is that clustering greedily merges a good pair of subsets without recognizing the global context of when either subset is to be scheduled. Hence, it misses several things including the ability to partially overlap (i.e., pipeline) the subsets. Dynamic promotions offer a form of pipelining but there is no guarantee that the most-useful-to-pipeline tasks will execute together. More fundamentally, while this algorithm does identify task subsets that pack well together, the constraint that there be no dependencies between tasks in any subset restricts the oppurtunities to pack better.

\subsection{Gv2: Top-down editing of cluster state}
\label{subsec:gv2}
In reaction to the inability of Gv1 to reason about global context, this approach emulates the execution of various scheduling algorithms, obtains the ensuing {\em cluster state} and edits the cluster state to improve job runtimes. The {\em cluster state} is a timestamped record of which task is scheduled to which machine and offers complete knowledge of where and when the tasks of a DAG run. We explored several types of edits~\xref{subsec:gv2_edits}. We use a large bag of scheduling algorithms including proposals from literature and Gv1~(\xref{subsec:gv1}).

This proposal has two potential advantages. First, by exploring many different ways to schedule the DAGs, it can pick the approach that works best. We find that among the baselines explored different algorithms worked better for different DAGs.  Second, it could potentially improve further by editing the schedule as described next.

\subsubsection{Edits}
\label{subsec:gv2_edits}
The goal of an edit is to improve job runtime. When multiple DAGs are involved, the goal is to improve average job completion time.  Our first type of edit matches unused resources with tasks that have been scheduled later.  That is, it identifies free {\em slots}, i.e., \{machine, time\_{begin}, time\_{end}, freeRsrcs\} tuples in the current cluster state and looks for tasks that could avail of these resources but happen to be scheduled later. Such a task has to satisfy three conditions: (a) all of the task's parents finish before the slot begins,  (b) the task's resource demands are below freeRsrcs, and (c) the anticipated duration of the task is smaller than the duration of the slot.  A second type of edit looks for pairs of tasks to swap that satisfies similiar constraints. The intuition is that  a short duration task scheduled next to a free slot can be swapped with a long running task that is scheduled at some later time.  We efficiently search for feasible edits, greedily rank them by their impact on job runtime, make the best edit and repeat until no more edits are feasible.

\subsubsection{Findings}
\label{subsec:gv2_drawbacks}
Such top-down editing works quite well at plugging the holes left by some of the less performant scheduling algorithms from literature. However, we find two key problems that limit the practical value of this approach beyond discovering the "best-of-breed" scheduling algorithm.  First, greedy scheduling algorithms that also allow for over-allocation~\xref{subsec:overallocation} do leave free slots, but neither are the free resources large enough nor are the durations long enough to allow for task promotions.  Oppurtunities to swap tasks are more frequent, however.  Second, the "edit distance" between the cluster state achieved by the best-of-breed schedalgo and a substantially better cluster state (e.g., with much smaller average job completion time) is often large; swapping a pair of tasks does not by itself improve job completion time but rather often requires many other dependent tasks to be promoted as well. Achieving all of these edits often requires reconfiguring triples, quadruples or larger sets of tasks-- a search space that can become quite large.

\subsection{Gv3: xxx}
\label{subsec:gv3}
Guided by the findings from developing the above two approaches, we realize that global context is important to schedule a DAG well, for resource packing and to ensure that critical path is not inflated. However, editing a candidate cluster state is not very useful due to the large edit distance between that state and the desired state.  This proposal constructs a good cluster state from first principles.

Since it is hard to construct the optimal schedule, let us think about how to verify whether some given schedule could be improved further.  If all the resources are fully utilized at all times during the execution of the DAG~(or judiciously over-utilized~\label{subsec:overalloc}), then the schedule is for sure optimal. Clearly, however, this does not always happen. DAGs may have "choke-points" with low degree of parallelism as in [insert figure] or they may only need a little for some resource. Hence, the verification has to also check that, whenever resources are under-used, nothing better could have been done. That is, no other ordering of tasks would use more of the resources during execution. Choke points can also be caused by tasks with {\em large} and {\em odd} resource demands that result in a lot of resource fragmentation. Similarly, tasks with long durations, if not scheduled carefully, lead to low degree of paralellism since their dependents cannot run until the tasks finish. It follows then that avoiding the most likely causes behind the under-use of resources could lead to a good schedule.

\subsubsection{algo}
Our method to avoid these most likely causes is as follows. First, identify the potentially problematic tasks, let this set be $P$. Second, identify the smallest connected component in the DAG that includes $P$ and call that $\hat{P}$. Third, schedule the tasks in $\hat{P}$ greedily while respecting any dependencies between the tasks in the set; the schedule will be represented as a cluster state. Fourth, divide the tasks not in $\hat{P}$ into two groups--call them {\em beforeP} and {\em afterP}. If the task has a descendant in $\hat{P}$, it falls into beforeP, else it falls into afterP. Fifth, schedule whichever of these two groups has more {\em work} first followed by the other.  When scheduling either group pack them as tightly as possible while allowing for overlaps onto the tasks in $\hat{P}$.  That is, when scheduling tasks in afterP, place the task with the longest expected duration (and/or resource demand), all of whose {\sf parents} have already been placed, at the {\sf earliest} possible location. This location can overlap with tasks in $\hat{P}$ as long as it happens after the last parent of the task being placed. Placing tasks with longer durations and/ or resource demands first ensures that the overall schedule will be tight. Similarly, when scheduling tasks in beforeP, place the longest task, all of whose {\sf children} have already been placed at the {\sf latest} possible location.

Identifying the potentially problematic tasks is tricky and the resultant schedule can crucially depend on the set that has been chosen. Hence, we perform a small search procedure that explores several threshold values (on the task duration, on the potential to cause resource fragmentation, etc.) and pick the best resultant schedule.

\subsubsection{findings}
over a large set of DAGs from production, this algorithm does better than all of the examined baselines.

\subsection{Judicious over-allocation of resources}
\label{subsec:overalloc}
Today's schedulers do not consider all the resources consumed by a task~(especially disk and network) during the assignment process which may lead to \textit{over-allocation} of these resources~\cite{tetris}. For example, if two tasks that can fully utilize the network are scheduled together, their completion time doubles.  Rampant over-allocation leads to poor performance since even though all of the resources appear utilized~(at 100\% usage for e.g.,) tasks are substantially delayed and collapse can happen~(e.g., too many seeks, memory thrashing, network incast).

Over-allocation is not always bad. When resources are constrained, it is often better to {\it slightly} over-allocate the fungible resources such as network and disk. Consider the following example: a scheduler which assigns tasks based on two resources: memory~(hard resource) and network~(fungible resource). Assume that each machine has the same capacity and each task requires 25\% memory and 40\% network~(percentages are over machine capacity).  Here, a machine can run two tasks at a time without over-allocation. If task duration is $1$, the per machine throughput is 2 tasks. However, if three tasks are scheduled simultaneously, network becomes over-allocated~(120\%) and the task duration increases to $1.2$. However, note that the per machine throughput is now $2.5$~($3 / 1.2$) tasks. Over-allocating further does not improve throughput. The key reason behind increase in throughput from slight over-allocation is that resources are being wasted otherwise due to fragmentation.

Over-allocation is not always useful. When other machines are free, it is better to schedule tasks on those machines rather than over-allocate. The reason is because over-allocation will increase task duration. 
%For example, consider two available machines and four tasks to schedule(same task profile as above), the cluster throughput is 4 units by spreading tasks. Over-allocating tasks on any machine is doing worse; allocating three tasks on a machine and one on the other machine leads to a total throughput of 3.33 units; assigning all four tasks to the same machine degrades it to 2.5 units. 
Similarly, if other tasks exist that can run without over-using the fungible resources, it is better to schedule them instead. 
%For example, given four tasks such as above, and four tasks that require 25\% memory and 0\% network, it is better to place two tasks that need network and two that do not, on each machine, for a machine throughput of 4 units. Placing any fewer tasks or running more tasks of the former or the latter type at any one time lowers the overall throughput. 

Packing schedulers such as Tetris never over-allocate~\cite{tetris}. Production schedulers ignore the network and disk demands~\cite{}. Hence, whenever the cluster is busy, Tetris is inefficient. Whenever tasks have heterogeneous usages of network or disk, prior schedulers are inefficient. Reduce tasks are typically much more network-intensive than maps. We show how to combine the best of both world when dealing with over-allocation. 

\subsubsection{algo}
Our goal is to determine whether to over-allocate. The algorithm has to work when tasks have different resource demands, durations and begin times.

When placing a task at a machine can lead to over-allocation we project into the future to compute the anticipated completion times of the new task as well as all the other tasks already running at that machine. If the task is not placed at this machine, it has two options (a) be placed on some other machine that has free resources now or (b) wait until some task finishes at any machine. We measure the {\em benefit} from overallocation as the difference between the completion time of the new task when placed with overallocation compared to the best possible completion time otherwise~(minimum of case (a) and (b)). Notice that, by definition of over-allocation, placing the new task would increase the completion times of the already running tasks. The {\em cost} from overallocation is measured as the sum of the increase in completion times of the tasks already running on this machine. Overallocation is allowed only if the benefit-- reduction in completion time of the task to be placed -- outweighs the cost -- total delay in other tasks.

\subsubsection{combining over-allocation with Gv3}
Recall that Gv3 places the problematic tasks first and then attempts to pack parents and children as tightly as possible. It is computationally expensive to use the above logic when computing the schedule with Gv3
since overallocation can violate the dependencies of tasks that have already been placed. Guaranteeing no violations implies no overallocation and may leave gains on the table. OTOH, fixing violations may require a cascade of tasks to be moved around. 

Instead we do the following. The above overallocation logic is employed by the dynamic scheduler. Hence, even when Gv3 computes schedules without overallocation, the actual scheduling of the DAG benefits from judicious allocation. In addition, when computing good schedules, Gv3 searches over a small number of over-allocation thresholds (e.g., 1, 1.05 and 1.1) wherein given a threshold, tasks are packed so that the maximum resource use never crosses the threshold. Threshold$=1$ implies no overallocation and $=1.1$ implies no more than 10\% overuse. When the threshold is small enough, we intuitively expect the ensuing schedule to be mostly correct since over-allocation leads to dependency violations only if a child (or parent) starts (or ends) right after (or before) the task impacted by over-allocation. We expect the gains in task throughput from over-allocation to more than offset the time lost to handle these violations on the forward path.


\subsection{Implementing {\name} in cluster schedulers}
Gv3 outputs per machine a sequence of tasks that can run on that machine.  This sequence is made available to the job managers (e.g., the YARN AM) and/or the cluster scheduler (e.g., the YARN RM). The job managers preferentially requests resources for these tasks and the cluster manager preferentially matches tasks to machines per this schedule.

In the ideal case, each task runs on the machine that it is supposed to run at.  But, what we do actually at  runtime is XXX

implementations are bound to differ from the actual schedule; how can we fix that?


==> texfiles/flowchart.tex <==
%!TEX root=../graphene.tex
\tikzstyle{startstop} = [rectangle, rounded corners, minimum width=1cm, minimum height=1cm,text centered, draw=black, fill=red!10]

\tikzstyle{io} = [trapezium, trapezium left angle=70, trapezium right angle=110, minimum width=1cm, minimum height=1cm, text centered, draw=black, fill=blue!30]


\tikzstyle{process} = [rectangle, minimum width=1cm, minimum height=1cm, text centered, draw=black, fill=orange!10]
\tikzstyle{decision} = [diamond, minimum width=1cm, minimum height=1cm, text centered, draw=black, fill=green!10]

\tikzstyle{arrow} = [thick,->,>=stealth]




\begin{tikzpicture}[node distance=0.05in]

\node (start) [draw=none,fill=none,text width=1in] {Packing and dependencies?};
\node (OnlyScheduling) [process, right of=start, xshift=2cm,text width=1in] {Only Dependencies (\cite{})};
\node (OnlyPacking) [process, left of=start, xshift= -2cm,text width=1in] {Only Packing \cite{tetris,reverse-fit,psv}};
\draw [arrow] (start) -- (OnlyPacking);
\draw [arrow] (start) -- (OnlyScheduling);
\node (RealisticModel) [draw=none,fill=none, below of=start, yshift= -2cm,text width=1in] {Realistic Model?};
\node (JobShop) [process, right of= RealisticModel, xshift=2cm,text width=1in] {Job Shop scheduling \cite{Czumaj:2000,Goldberg:1997,Shmoys:1994}, strip packing \cite{StripPart, ChekuriK04,AzarCG13} };
\node (StochasticScheduling) [process, left of= RealisticModel, xshift= -2cm,text width=1in] {Stochastic Scheduling \cite{algo_pack_precedence3}};
\draw [arrow] (RealisticModel) -- (JobShop);
\draw [arrow] (RealisticModel) -- (StochasticScheduling);
\draw [arrow] (start) -- (RealisticModel);

\node (Cluster) [draw=none,fill=none, below of=RealisticModel, yshift= -2cm,text width=1in] {Practical In Clusters?};
\node (ILP) [process, right of= Cluster, xshift=2cm,text width=1in] {ILP, Configuration LP};
\node (VMAlloc) [process, left of= Cluster, xshift= -2cm,text width=1in] {VM allocation \cite{Chowdhury2009a}};
\draw [arrow] (Cluster) -- (ILP);
\draw [arrow] (Cluster) -- (VMAlloc);
\draw [arrow] (RealisticModel) -- (Cluster);

\node (Fairness) [draw=none,fill=none, below of=Cluster, yshift= -2cm,text width=1in] {Fairness?};
\draw [arrow] (Cluster) -- (Fairness);
\end{tikzpicture}



==> texfiles/intro_aditya.tex <==
%!TEX root=../graphene.tex 

\section{Introduction} 
\label{sec:intro} 

Commercial enterprises increasingly use a data-driven approach to make
business decisions. Using scale-out clusters to store and analyze data has become 
commonplace. Such clusters were initially popularized by
Map-Reduce~\cite{mapreduce} jobs but have now evolved to support generic
programming models~\cite{presto,scopestreaming,blinkdb} 
leading to more complex queries~\cite{sparksql,scope-vldb12,dryad,tez,hive,flumejava}. 
In all these frameworks a job is represented as a {\em directed acyclic graph~(DAG) of tasks}.

Scheduling these jobs efficiently is non-trivial, because of the
complexity in DAG structure, as well as diversity in resource demands
of their constituent tasks.  Indeed, our analysis of a large
collection of production DAGs corresponding to SCOPE queries in
Microsoft's clusters
shows that the median job has a DAG of depth $6$ and about $10^3$
tasks! The DAGs come in different shapes, too. Some are long chains;
most are not trees. \aditya{inverted tree?}% The DAG
% structure primarily reflects query complexity. The DAG size is roughly
% proportional to the size of input times the passes needed by the
% computation.  For e.g., joining two large tables is a DAG of depth
% $3$~(1:partition on join key, 2:shuffle, 3:join) wherein each level
% has enough tasks to process the data in parallel.
Further,%  tasks have very different demands for resources such as CPU,
% memory, disk and network%
we observe a high ($\sim1$)
coefficient-of-variation~(${\mbox{stdev.}}/{\mbox{avg.}}$) for many
resources, including CPU, memory, disk and network. \aditya{what are
  the stddev and average computed over?}  These are arising due to differences
in user code~(e.g., machine learning tasks hog CPU and memory) and due
to nuances of the underlying data-parallel framework~(e.g., only
shuffles are network intensive). \aditya{I don't get the last point}

% Given the size and capital invested in these clusters, improving scheduling
% efficiency by even $10$\% in production is a sizable win. \fixme{more?}

State-of-the-art proposals fall seriously short in scheduling such
jobs effectively. For instance, recent work on packing tasks carefully
along multiple resources~\cite{tetris,vector} can let more tasks run
simultaneously, potentially improving cluster throughput and finishing
jobs quicker. However, dependencies between tasks substantially
complicates packing.  First there is a mismatch between two
optimization objectives-- the best-packed task may not be the task
with the longest critical path of the job's DAG. Hence, focusing only
on packing will cause lulls on critical path, leading to resource
waste and slowdown. Second, since tasks are schedulable only when
their dependencies are met, the subset that will be schedulable at a
time depends on earlier scheduling decisions. Hence, local packing
decisions that only examine currently schedulable tasks are much worse
than global decisions that consider the entire DAG. Indeed, we show
that state-of-the-art packers~\cite{tetris,vector} can be $d\times$
worse than optimal when used to schedule DAGs, where $d$ is the number
of relevant resources ($d=4$ in practice).

On the other hand, available critical path scheduling algorithms for
DAGs~\cite{coffman-graham} are not effective either because they
assume tasks have homogeneous demands. When tasks have varying
demands, we show that these algorithms are up to $O(n)\times$ worse
than optimal, where $n$ is the number of tasks in the DAG.

Finally, production cluster schedulers, which are far more simplistic than DAG
schedulers or packers, schedule based on exogenous factors such as
disk locality and fairness. An analysis of the completion times of the
SCOPE jobs at Microsoft's clusters shows runtimes $2\times$ larger than a lower bound
for half the DAGs and $4\times$ larger for $25$\% of DAGs.

This paper presents the design, implementation, and evaluation of,
{\name}, an efficient scheduler that packs multiple resources for
concurrently executing multi-stage DAGs. Individually, both packing
and dependency-aware scheduling are NP hard problems~\cite{apx}.
\fixme{after theory talk} Thus, {\name} incorporate several carefully
designed heuristics. {\name} builds on two main ideas: identifying
important tasks that critically determine overall schedule efficacy,
and scheduling these first while avoiding deadlocks for other tasks;
and computing a global schedule that considers entire DAGs of all jobs
(as opposed to making greedy locally-optimal decisions).

\aditya{need a two sentence summary of the main ideas here?}

In more detail, our system, {\name}\footnote{For an allotrope of
  carbon that has a nice compact structure.}, works as
follows. Imagine a job's schedule to be a mapping of its tasks into
$d+1$ dimensional space~($d$ resource dimensions and time). To be
feasible, this mapping has to respect resource capacity limits and
inter-task dependencies. Among feasible schedules, the most compact
mapping has the smallest completion time. Given this setup, {\name}
assigns the {\em troublesome} tasks---those with long durations or
peculiarly shaped resource demands---first. Doing so helps in two
ways. (1) Since the space is relatively free initially, troublesome
tasks can be arranged compactly. (2) The remaining less-troublesome
tasks can be placed into the holes left after placing these
troublesome tasks.

However, mapping tasks on to the above space~(i.e., resources and
time) in arbitrary order leads to deadlocks. For example, if two tasks
are mapped, say because they were considered troublesome, then there
may not remain enough space for other tasks that lie between these two
tasks in the DAG.  Keeping some slack can help, but it is apriori
unclear how much space should be set aside.  Moreover, setting aside
too much would hurt compactness.  To address these issues, {\name}
maps tasks onto space in a careful order that guarantees no deadlocks.
Since more than one deadlock-free order exists, {\name} explores
multiple choices for troublesome tasks using a novel, efficient
strategy.

Furthermore, the schedule constructed above is per job. But, many jobs
run simultaneously on the cluster. The resources available to a job
change dynamically. And, there will be new arrivals, stragglers and
failures. Hence, {\name} decouples detailed schedule construction from
the enforcement.  Schedules are constructed offline at job submission
using historical statistics from similar jobs. At runtime, {\name}
adapts to dynamic changes and simultaneously enforces the desired
schedules of all the jobs running in the cluster.  Uniquely, the
online component offers (a) careful overbooking of resources and (b)
bounds unfairness. \fixme{explain each} We are not aware of any such
online scheduler. % Tetris~\cite{tetris} cannot enforce a desired DAG
% schedule, does not overbook, and leads to arbitrary amounts of
% unfairness.


%  by (a) cutting
% a DAG such that there is no overlap in schedule between the parts which allows
% picking the best possible lower bound per part and (b) accounting for
% parallelism better. \fixme{say better} We apply this new bound to over $20$K DAGs
% seen in production at Bing. Our analysis shows that {\name} is within $5$\% of
% the optimal for over half these DAGs.

We built an initial implementation for {\name} as extensions to Apache
YARN and Apache Tez framewrorks.  We extend the Tez~\cite{tez} job
manager to invoke the per DAG schedule construction algorithm. We
extend the RM~(resource manager) in Yarn~\cite{yarn} to implement the
online component of {\name}.  Many of our extensions have been
subsequently committed back to these open source projects.
\aditya{check this} % The baseline
% schedulers in Yarn, capacity- and fair- schedulers, both greedily
% assign a task with good data locality from among the queue that is
% currently most under-served. With {\name}, the logic of both
% schedulers remains identical except for: (a) they pick a task per
% desired schedule for DAG, (b) they prefer jobs with less remaining
% work, (c) they overbook resources and (d) relax fairness for
% performance yet the extent of unfairness is bounded. 
We evaluated our
prototype on a $200$ server cluster using queries from a variety of
benchmarks including TPC-DS\cite{tpc-ds} and TPC-H~\cite{tpc-h}. 

Our key experimental findings are:
\begin{Itemize} 
\item Relative to Tez,
{\name} improves completion time of half of the DAGs by $19-31$\% across the
various benchmarks. A quarter of the DAGs improve by $30-49$\%. Relative to Tetris and 
Critical path, {\name} improves by $15-40$\%. 
\item From analyzing $20$K production DAGs from
Bing, the schedules constructed by {\name} are $25$\% faster for half the DAGs.
A quarter improve by $57$\%. 
% \item By applying our new lower bound, we show that
% {\name}'s schedules are optimal for $40$\% of DAGs.
% Three quarters of the DAGs are within $13$\%.
\end{Itemize}

\aditya{nothing about fairness above?}

The optimal packing+dependencies solution is intractable to compute
and the available lower bounds are loose~\cite{StripPart}. We develop
a much tighter lower bound and, through our experiments, find that
{\name}'s schedules are optimal for $40$\% of DAGs, and that three
quarters of the DAGs are within $13$\%.


To summarize, the key contributions of {\name} are: 
\begin{Itemize} 
\item A
novel DAG scheduling algorithm that packs tasks along multiple resources and
time while respecting dependencies. 
\item An online component that
(softly) achieves the desired schedule order for all the DAGs in the cluster. \aditya{something about fairness?}
\item A new much tighter lower bound on the completion time of a DAG of tasks.
\item An implementation that has been checked in to Apache
  Yarn\footnote{put the JIRA here},
  extensive experiments with Tez and Hive jobs on a cluster, and
  extensive analysis of the DAGs in production SCOPE jobs at
  Bing. 

\end{Itemize}

Similar packing+dependencies scheduling problems arise elsewhere
too. We offer early results from applying {\name} to scheduling the
DAGs in distributed build systems~\cite{bazel,cloudmake} and
request-response workflows~\cite{kwiken}. \fixme{cya}
\aditya{I think we should take this out entirely}


==> texfiles/introduction.tex <==
%!TEX root=../graphene.tex 

\section{Introduction} \label{sec:intro} Commercial enterprises increasingly use
a data-driven approach to make business decisions. Clusters that initially ran
Map-Reduce~\cite{mapreduce} jobs now offer more generic programming models to
support interactive queries~\cite{presto,scopestreaming,blinkdb} and more
complex ad-hoc queries~\cite{sparksql,scope-vldb12,dryad,tez,hive,flumejava}. In
all these frameworks a job is represented as a directed acyclic graph~(DAG) of
tasks.

Examining production SCOPE queries at Bing, we find that job DAGs are deep, with
many tasks and have many different shapes. Some are long chains. Most are not
trees. The median job has a depth of $6$ and has $O(10^3)$ tasks. The DAG
structure primarily reflects query complexity. The DAG size is roughly
proportional to the size of input times the passes needed by the computation.
For e.g., joining two large tables is a DAG of depth $3$~(1:partition on join
key, 2:shuffle, 3:join) wherein each level has enough tasks to process the data
in parallel.

Further, tasks have very different demands for resources such as CPU, memory,
disk and network. The coefficient-of-variation~(${\mbox{stdev.}}/{\mbox{avg.}}$)
is about $1$ for many resources. This variability arises due to user code~(e.g.,
machine learning tasks hog CPU and memory) and due to the data-parallel
framework~(e.g., only shuffles are network intensive).

Given the size and capital invested in these clusters, improving scheduling
efficiency by even $10$\% in production is a sizable win. \fixme{more?}


Packing tasks carefully along multiple resources lets more tasks run
simultaneously. In turn, this improves cluster throughput and finishes jobs
quicker. However, dependencies between tasks substantially complicates packing.
First there is a mismatch between two optimization objectives-- the best-packed
task may not be the task with the longest critical path. Hence, focusing only on
packing will cause lulls on critical path. Second, since tasks are schedulable
only when their dependencies are met, the subset that will be schedulable at a
time depends on earlier scheduling decisions. Hence, local packing decisions
that only examine currently schedulable tasks are much worse than global
decisions that consider the entire DAG. Due to these reasons, we show that
packers~\cite{tetris,vector} can be $d\times$ worse than optimal when
used to schedule DAGs. Here $d$ is the number of relevant resources. It is about
$4$ in practice. Third, available DAG scheduling
algorithms~\cite{coffman-graham} assume tasks have homogeneous demands. When
tasks have varying demands, we show that these algorithms are up to $O(n)\times$
worse than optimal. Here, $n$ is the number of tasks in the DAG. Individually,
both packing and dependency-aware scheduling are NP hard problems~\cite{apx}.
\fixme{after theory talk}

Production cluster schedulers schedule based on exogenous factors such as disk
locality and fairness. An analysis of the completion times of the SCOPE jobs at
Bing shows runtimes $2\times$ larger than a lower bound for half the DAGs and
$4\times$ larger for $25$\% of DAGs.

\vskip .05in This paper offers new algorithms that pack multiple resources for
concurrently executing multi-stage DAGs.

\vskip .05in The key intuition behind our system, {\name}\footnote{For an allotrope of
carbon that has a nice compact structure.}, is as follows. Imagine a job's
schedule to be a mapping of its tasks into $d+1$ dimensional space~($d$ resource
dimensions and time). To be feasible, this mapping has to respect resource
capacity limits and inter-task dependencies. Among feasible schedules, the most
compact mapping has the smallest completion time. Given this setup, {\name}
assigns the troublesome tasks-- those with long durations or peculiarly shaped
resource demands-- first. Doing so helps in two ways. (1) Since the space is
relatively free initially, troublesome tasks can be arranged compactly. (2) The
remaining less-troublesome tasks can be placed into the holes left after placing
these troublesome tasks.

Several challenges remain. First, mapping tasks on to the above space~(i.e.,
resources and time) in arbitrary order leads to deadlocks. For example, if two
tasks are mapped, say because they were considered troublesome, then there may
not remain enough space for other tasks that lie between these two tasks in the DAG. 
Keeping some slack can help. But it is
apriori unclear how much space should be set aside. And, setting aside too much
would hurt compactness. {\name} maps tasks onto space in a careful
order that guarantees no deadlocks.

Second, more than one deadlock-free order exists. As well, {\name} explores
different choices for troublesome tasks since it is apriori unclear which tasks
will be troublesome. {\name} uses an efficient strategy to search among the
various alternatives.

Third, the schedule constructed above is per job. But, many jobs run
simultaneously on the cluster. The resources available to a job change
dynamically. And, there will be new arrivals, stragglers and failures. Hence, {\name}
decouples detailed schedule construction from the online enforcement. 
Schedules are constructed at job submission using historical statistics from similar 
jobs. At runtime, {\name} adapts to dynamic changes and
simultaneously enforces the desired schedules of all the jobs running in the
cluster.

Uniquely, the online component offers (a) careful overbooking of resources and
(b) bounds unfairness. \fixme{explain each} We are not aware of any such online
scheduler. Tetris~\cite{tetris} cannot enforce a desired DAG schedule, does not
overbook, and leads to arbitrary amounts of unfairness.

Finally, the optimal packing+dependencies solution is intractable to compute and
the available lower bounds are loose~\cite{StripPart}. Hence, it was impossible to determine the
gap from optimality. We develop a new much tighter lower bound by (a) cutting
a DAG such that there is no overlap in schedule between the parts which allows
picking the best possible lower bound per part and (b) accounting for
parallelism better. \fixme{say better} We apply this new bound to over $20$K DAGs
seen in production at Bing. Our analysis shows that {\name} is within $5$\% of
the optimal for over half these DAGs.

We built a substantial prototype for {\name}. Much of the prototype has been
committed back to the relevant open source projects. We extend the
Tez~\cite{tez} job manager to invoke the per DAG schedule construction
algorithm. We extend the RM~(resource manager) in
Yarn~\cite{yarn}. The baseline schedulers in Yarn, capacity- and fair-
schedulers, both greedily assign a task with good data locality from among the
queue that is currently most under-served. With {\name}, the logic of both
schedulers remains identical except for: (a) they pick a task per desired
schedule for DAG, (b) they prefer jobs with less remaining work, (c) they overbook
resources and (d) relax fairness for performance yet the extent of unfairness is
bounded. We evaluated our prototype on a $200$ server cluster using queries from
a variety of benchmarks including TPC-DS\cite{tpc-ds} and TPC-H~\cite{tpc-h}. Our
key findings are: 
\begin{Itemize} 
\item Relative to Tez,
{\name} improves completion time of half of the DAGs by $19-31$\% across the
various benchmarks. A quarter of the DAGs improve by $30-49$\%. Relative to Tetris and 
Critical path, {\name} improves by $15-40$\%. 
\item From analyzing $20$K production DAGs from
Bing, the schedules constructed by {\name} are $25$\% faster for half the DAGs.
A quarter improve by $57$\%. 
\item By applying our new lower bound, we show that
{\name}'s schedules are optimal for $40$\% of DAGs.
Three quarters of the DAGs are within $13$\%.
\end{Itemize}

To summarize, the key contributions of {\name} are: 
\begin{Itemize} 
\item A
novel DAG scheduling algorithm that packs tasks along multiple resources and
time while respecting dependencies. 
\item An online component that
(softly) achieves the desired schedule order for all the DAGs in the cluster.
\item A new much tighter lower bound on the completion time of a DAG of tasks.
\item An implementation that has been checked in to Apache Yarn.
Extensive experiments with Tez and Hive jobs on a cluster. And extensive
analysis of the DAGs in production SCOPE jobs at Bing. \end{Itemize}

Similar packing+dependencies scheduling problems arise elsewhere too. We offer
early results from applying {\name} to scheduling the DAGs in distributed build
systems~\cite{bazel,cloudmake} and request-response workflows~\cite{kwiken}. \fixme{cya}

==> texfiles/introv2.tex <==
%!TEX root=../graphene.tex 

\section{Introduction} 
\label{sec:intro} 

Commercial enterprises increasingly use a data-driven approach to make
business decisions. Using scale-out clusters to store and analyze data has become 
commonplace. Such clusters were initially popularized by
Map-Reduce~\cite{mapreduce} jobs but have now evolved to support generic
programming models~\cite{presto,blinkdb,scopestreaming} 
leading to more complex queries~\cite{tez,sparksql,flumejava,dryad,hive,scope-vldb12}. 
In all these frameworks a job is represented as a {\em directed acyclic graph}~(DAG) of tasks.


Scheduling these jobs efficiently is non-trivial because of the
complex DAG structure and the diversity in resource demands
of the constituent tasks.  Indeed, our analysis of a large
collection of production DAGs corresponding to SCOPE queries in
Microsoft's clusters
shows that the median job has a DAG of depth $7$ and $10^3$
tasks! The DAGs come in different shapes, too (see Fig.~\ref{fig:egdags}) and most DAGs are not trees. The DAG structure is complex primarily because the 
underlying queries do interesting things. The DAGs
are the outputs of a query optimizer which converts a user query into a 
performant plan for parallel execution.
% The DAG
% structure primarily reflects query complexity. The DAG size is roughly
% proportional to the size of input times the passes needed by the
% computation.  For e.g., joining two large tables is a DAG of depth
% $3$~(1:partition on join key, 2:shuffle, 3:join) wherein each level
% has enough tasks to process the data in parallel.
Further,
across all tasks that ran in a cluster
%  tasks have very different demands for resources such as CPU,
% memory, disk and network%
we observe a high ($\sim1$)
coefficient-of-variation~(${\mbox{stdev.}}/{\mbox{avg.}}$) for many
resources, including CPU, memory, disk and network.
These arise due to differences
in user code~(e.g., machine learning tasks hog CPU and memory) and 
the different roles of the tasks~(e.g., shuffle tasks are network intensive).

% Given the size and capital invested in these clusters, improving scheduling
% efficiency by even $10$\% in production is a sizable win. \fixme{more?}

State-of-the-art proposals fall seriously short in scheduling such
jobs effectively. For instance, recent work on packing tasks along multiple 
resources~\cite{tetris,vector} lets more tasks run
simultaneously which in turn improves cluster throughput and
job completion times. However, dependencies between tasks substantially
complicates packing.  First, there is a mismatch between two
optimization objectives---the best-packed task may not be the task
with the longest critical path on the job's DAG. Hence, focusing only
on packing will cause lulls on critical path.
%, leading to resource waste and slowdown. 
Second, since tasks are schedulable only when
their dependencies are met, the subset that will be schedulable at a
time depends on earlier scheduling decisions. Hence, local packing
decisions that only examine currently schedulable tasks can make inefficient
choices compared to global decisions that consider the entire DAG. Indeed, we show
that state-of-the-art packers~\cite{tetris,vector} can be $d\times$
worse than the optimal when used to schedule DAGs, where $d$ is the number
of relevant resources ($d=4$ in practice).

\begin{figure}[t!]
\centering
\includegraphics[width=2in]{figures/egdags.png}
\ncaption{Common DAG patterns in production jobs. A circle denotes a stage consisting of 
one or more tasks. Map-reduce jobs have a two-stage DAG with a shuffle between the 
corresponding tasks.\label{fig:egdags}}
\end{figure}
On the other hand, available critical path scheduling algorithms for
DAGs~\cite{coffman-graham} are not effective either, because they
assume tasks have homogeneous demands. When tasks have varying
demands, we show that these algorithms are up to $n\times$ worse
than optimal, where $n$ is the number of tasks in the DAG.

Finally, production cluster schedulers, which tend to be simpler than the above mentioned DAG
schedulers or packers, schedule based on exogenous factors such as
disk locality and fairness. An analysis of the completion times of the
SCOPE jobs at Microsoft's clusters shows runtimes $2\times$ larger than a lower bound
for half the DAGs and $4\times$ larger for $25$\% of DAGs.

This paper presents the design, implementation, and evaluation of,
{\name}\footnote{For an allotrope of
  carbon that has a compact structure.}, an efficient scheduler that packs multiple resources for
concurrently executing multi-stage DAGs. Individually, both packing
and dependency-aware scheduling are NP hard problems~\cite{apx}.
Thus, {\name} incorporates several carefully
designed heuristics. 

{\name} uses the following main idea for schedule construction: 
identify important tasks that critically 
determine overall schedule efficacy and schedule those first, while 
avoiding deadlocks for other tasks. In doing so, {\name} 
computes a global schedule that considers the entire DAG of a job
as opposed to making greedy locally-optimal decisions.

In more detail, 
some tasks are potentially more troublesome than others.
For example, long-running tasks can adversely impact the overall schedule 
if tasks that could have run alongside these tasks were executed early.
{\name} first maps the troublesome tasks onto a 
$d+1$ dimensional space~($d$ resource dimensions and time).
Since the space is relatively free initially, these
tasks can be arranged compactly. Subsequently, the remaining tasks can be 
packed into the resource-time holes left after placing the
troublesome tasks. However, the above order can lead to deadlocks.  For example, if two tasks
are mapped because they were considered troublesome then there
may not remain enough space for tasks that lie between these two
tasks in the DAG. 
A simple strawman approach of leaving some slack space apriori 
is inefficient since it is unclear how much should be set aside.
{\name} shows how to map tasks onto the resource-time
space without deadlocks.

\vskip .05in
{\name} decouples the above described schedule construction from online packing and 
fairness guarantees. 
Schedules are constructed per job using historical statistics.
Recurring jobs can reuse pre-constructed schedules.
The online component enforces the desired schedules of the various DAGs.
In addition, {\name} offers a new packing heuristic that overbooks resources
judiciously. 
Furthermore, for a wide variety of desirable fairness schemes, {\name} 
improves performance while bounding the extent of unfairness.
That is, given a threshold $\kappa$, {\name} ensures that the gap from desired
fair share~(of cluster resources) never dips below $\kappa C$ where $C$ is cluster
capacity.
We are not aware of any such online scheduler for data-parallel clusters.
%Both these aspects are novel for a data-parallel scheduler

\eat{
In more detail, our system, {\name}, works as
follows. Imagine a job's schedule to be a mapping of its tasks into
$d+1$ dimensional space~($d$ resource dimensions and time). To be
feasible, this mapping has to respect resource capacity limits and
inter-task dependencies. Among feasible schedules, the most compact
mapping has the smallest completion time. Given this setup, {\name}
assigns the {\em troublesome} tasks---those with long durations or
peculiarly shaped resource demands---first. Doing so helps in two
ways. (1) Since the space is relatively free initially, troublesome
tasks can be arranged compactly. (2) The remaining less-troublesome
tasks can be placed into the holes left after placing these
troublesome tasks.

However, mapping tasks on to the above space~(i.e., resources and
time) in arbitrary order leads to deadlocks. For example, if two tasks
are mapped, say because they were considered troublesome, then there
may not remain enough space for other tasks that lie between these two
tasks in the DAG.  Keeping some slack can help, but it is apriori
unclear how much space should be set aside.  Moreover, setting aside
too much would hurt compactness.  To address these issues, {\name}
maps tasks onto space in a careful order that guarantees no deadlocks.
Since more than one deadlock-free order exists, {\name} explores
multiple choices for troublesome tasks using a novel, efficient
strategy.

Furthermore, the schedule constructed above is per job. But, many jobs
run simultaneously on the cluster. The resources available to a job
change dynamically. And, there will be new arrivals, stragglers and
failures. Hence, {\name} decouples detailed schedule construction from
the enforcement.  Schedules are constructed offline at job submission
using historical statistics from similar jobs. At runtime, {\name}
adapts to dynamic changes and simultaneously enforces the desired
schedules of all the jobs running in the cluster.  Uniquely, the
online component offers (a) careful overbooking of resources and (b)
bounds unfairness. \fixme{explain each} We are not aware of any such
online scheduler. % Tetris~\cite{tetris} cannot enforce a desired DAG
% schedule, does not overbook, and leads to arbitrary amounts of
% unfairness.
}

\vskip .05in
How good is {\name}?
The optimal packing+dependencies solution is intractable to compute.
And, the available lower bounds are very loose~\cite{StripPart}. We develop
a new bound that is tighter by about $30$\%.  Using this new bound, we show that
{\name}'s schedules are optimal for $40$\% of DAGs and within $13$\% for $75$\% 
of the DAGs.

%  by (a) cutting
% a DAG such that there is no overlap in schedule between the parts which allows
% picking the best possible lower bound per part and (b) accounting for
% parallelism better. \fixme{say better} We apply this new bound to over $20$K DAGs
% seen in production at Bing. Our analysis shows that {\name} is within $5$\% of
% the optimal for over half these DAGs.

We implemented {\name} by extending the Apache YARN~\cite{yarn} 
and Apache Tez~\cite{tez} 
frameworks. Schedule construction happens in the extended Tez job
manager. The extended YARN RM~(resource manager) implements 
schedule enforcement, packing, overbooking and bounded unfairness.
We are in the process of committing these changes to open source.
Several substantial aspects have been committed already.
% The baseline
% schedulers in Yarn, capacity- and fair- schedulers, both greedily
% assign a task with good data locality from among the queue that is
% currently most under-served. With {\name}, the logic of both
% schedulers remains identical except for: (a) they pick a task per
% desired schedule for DAG, (b) they prefer jobs with less remaining
% work, (c) they overbook resources and (d) relax fairness for
% performance yet the extent of unfairness is bounded. 
We evaluated our
prototype on a $200$ server cluster using queries from TPC-DS\cite{tpc-ds}, TPC-H~\cite{tpc-h}
and the DAGs seen in production at Bing.


\vskip .05in
To summarize, the key contributions of {\name} are: 
\begin{Itemize} 
\item A
novel DAG scheduling algorithm that packs tasks along multiple resources and
time while respecting dependencies~(\xref{sec:design}). 
\item An online component that
(softly) achieves the desired schedule order for all the DAGs in the cluster. 
The online component guarantees bounded unfairness and packs with careful overbooking~(\xref{sec:runtime}).
\item A new much tighter lower bound on the completion time of a DAG of tasks~(\xref{sec:betterlb}).
\item An implementation that has been partially checked in to relevant Apache 
projects~(\xref{sec:system}), 
extensive experiments with Tez and Hive jobs on a cluster,  
and extensive analysis of the DAGs in production SCOPE jobs at Bing. 
\item Relative to Tez,
{\name} improves completion time of half of the DAGs by $19-31$\% across the
various benchmarks. A quarter of the DAGs improve by $30-49$\%. Relative to Tetris and 
Critical path, {\name} improves by $15-40$\%. The improvements
for production Bing DAGs are larger~(half the DAGs speed up by $25$\%
and a quarter by $57$\%) because they have more user-defined code and varying 
resource demands~(\xref{sec:eval}).
%\item From analyzing $20$K production DAGs from
%Bing, the schedules constructed by {\name} are $25$\% faster for half the DAGs.
%A quarter improve by $57$\%. 
% \item By applying our new lower bound, we show that
% {\name}'s schedules are optimal for $40$\% of DAGs.
% Three quarters of the DAGs are within $13$\%.
\end{Itemize}

In what follows, we first outline the problem of packing with dependencies 
for DAGs~(\xref{sec:packdeps}).  We then provide an analysis of DAGs from Microsoft's
production clusters~(\xref{sec:background}) and then present {\name} system.

\eat{
Similar packing+dependencies scheduling problems arise elsewhere
too. We offer early results from applying {\name} to scheduling the
DAGs in distributed build systems~\cite{bazel,cloudmake} and
request-response workflows~\cite{kwiken}. \fixme{cya}
}


==> texfiles/introv3.tex <==
%!TEX root=../graphene.tex 

\section{Introduction} 
\label{sec:intro} 
Scale-out clusters are now commonly used to store and analyze large datasets.
%Overall, the above-mentioned cluster schedulers run on nearly a million servers today~\cite{bigDataPredictions}. 
For instance, several large enterprises (such as, Google, Yahoo, Ebay, Microsoft, Facebook, etc.) have private data-analytics clusters~\cite{bdas2}; many cloud providers (such as, Amazon AWS, Microsoft Azure, Google Compute Engine etc.) offer data analytics as a service~\cite{bdas}. 
These clusters now support complex programming models~\cite{tez,presto,blinkdb,sparksql,scopestreaming,flumejava,dryad,hive,scope-vldb12} 
due to which jobs have evolved from map tasks followed
by reduce tasks~\cite{mapreduce} to rich directed acyclic graphs~(DAGs) of tasks.
% To facilitate learning over massive datasets and data-driven business decisions, 
%See Fig.~\ref{fig:graphene_overview} for an example.

Scheduling these jobs efficiently is non-trivial because of the
complex DAG structure and the diverse resource needs
of the constituent tasks.  
Our analysis of production DAGs from a large enterprise finds that the median job has a DAG of depth $7$ and $10^3$ tasks. Several publicly available benchmarks such as TPC-H~\cite{tpc-h} and TPC-DS~\cite{tpc-ds} also have similarly complex DAGs.
The non-trivial DAG structures arise because the jobs perform complex analysis such as multi-way joins.  
% multiple inputs per job, complex analysis, and multiple outputs. 
% Furthermore, the DAGs are generated by an optimizer that looks for performant parallel plans.
Complicating matters even more, tasks in the cluster have diverse resource demands.
We observe a high~({\raise.17ex\hbox{$\scriptstyle\mathtt{\sim}$}}1) coefficient-of-variation~(stdev./avg.) for several resources. Such diversity is due to differences in user code and task roles. For example, machine learning tasks typically hog memory whereas, reduce tasks typically require data shuffling over the network.

Production cluster schedulers~\cite{tez,yarn,apollo,omega} schedule based on exogenous factors such as 
locality and fairness. Our analysis shows that $50$\% of the production DAGs in the examined clusters have runtimes two times larger than a lower bound. Because the problem of packing tasks with precedence constraints is NP-hard~\cite{MastrolilliS:2009}, we are unable to compute optimal completion times even for the case when each DAG runs by itself. Hence, we compare with a new lower bound that we have developed which is empirically much larger than the previously known bounds~\cite{StripPart,Mastrolilli:2008}. % on the examined DAGs.
%$25$\% of DAGs are off by $4\times$. 
%Tetris and critical path scheduling are off by $x$\% and $y$\% respectively  for $50$\% of the DAGs.

%A large body of algorithmic work considers the problem of packing+scheduling~\cite{}. We will discuss them at length later; however most of the results are about (1) hardness: there exist no algorithms with bounded competitive ratios

Most practical proposals  fail to achieve good performance because they either focus only on multi-resource packing~\cite{tetris,vector} or only on the precedence constraints~\cite{coffman-graham,graham}. We will call these algorithms {\em packers} and {\em DAG schedulers} respectively. Packers typically have heuristics to determine the best-packed task and greedily schedule that task next. Such local greedy choices often do not lead to a good {\em global} packing for the entire DAG. DAG schedulers typically schedule tasks based on the length of their critical path. They assume tasks have homogenous demands. Let $n$ and $d$ be the number of tasks in a DAG and the number of resources needed by each task. We show that (a) DAG schedulers can be up to $n$ times optimal when tasks have varying demands and (b) {\em any algorithm} that ignores dependencies, a class that includes the packers mentioned above, will be $d$ times optimal. Typical values for $d$ and $n$ are $4$ and a few hundred respectively; hence the worst-case performance of packers and DAG schedulers is very poor. In practice, we will show that both classes of algorithms are about $1.5$ times worse. Our metrics of interest are the average completion time of jobs and the cluster-wide job throughput~(e.g., makespan).


\begin{figure}[t!]
\centering
\includegraphics[width=3in]{figures/graphene_overview.png}
\ncaption{Shows steps taken by {\name} from a DAG on the left to its schedule on the
right. Each small circle is a stage with many tasks. Troublesome tasks~${\tt T}$~(in red) are placed
first. The rest of the subsets~(parents~${\tt P}$, children~${\tt C}$ and other~${\tt O}$) 
are placed {\em on top} of ${\tt T}$ in a careful order that ensures compactness and respects
dependencies.\label{fig:graphene_overview}}
\end{figure}

Improving cluster utilization by even a few percentage points can reduce the cost-of-operations considerably since more jobs can be supported without buying more servers. Furthermore, speeding up jobs can shorten the lag between data collection and decisions which potentially increases revenue~\cite{velocityLatency}.

Motivated by these observations, we design and implement {\name}, a cluster scheduler that combines multi-resource packing with dependency awareness. 

{\name} has two components.  First, at job submission time or soon thereafter, {\name}'s offline component builds a preferred schedule for tasks in that job. 
%The preferred schedule is an ordering over the tasks that leads to a compact global packing for the entire DAG. 
{\name} reuses previously computed preferred schedules for recurring jobs~\cite{rope}. Second, {\name} has an online component that enforces the preferred schedules of all the jobs running concurrently in the cluster. The online component also overbooks resources and improves performance
by trading-off a bounded amount of unfairness for many desirable fairness models (e.g., ~\cite{yarnFS,kellyPF,drf}).
% shows how to improve performance while bounding the extent of unfairness. 

\cut{
\vskip .05in
If there was only one resource and no dependencies, any work-conserving scheduler would do reasonably.  Because state-of-the-art proposals do either multi-resource packing or dependency-aware scheduling, they  fail to achieve good performance.
%
%By doing only one of the two-- multi-resource packing or dependency-aware scheduling--state-of-the-art proposals fall short.
For instance, packers~\cite{tetris,vector} greedily pick the best-packed task and ignore dependencies.  However, the best-packed task need not have the longest critical path. And, local greedy choices are unlikely to lead to a good {\em global} packing for the entire DAG. In fact, we show that {\em any scheduler} that ignores dependencies will be $\Omega(d)\times$ optimal when tasks need $d$ resources.\footnote{ 
In practice, there are at least four resources~(cores, memory, network and disk), i.e., $d\geq 4$.}
%Tetris is at least $(d+1)\times$ away. 
On the other hand, dependency-aware schedulers~\cite{coffman-graham,graham} assume tasks have homogeneous demands. We show that: when tasks have varying demands, by not packing, these algorithms are up to $n\times$ optimal,  where $n$ is the number of tasks in the DAG. Typically, $n\geq 100$~\cite{rope,mantri}.

Finally, production cluster schedulers~\cite{tez,yarn} schedule based on exogenous factors such as 
locality and fairness. Our analysis shows that $50$\% of the DAGs in Microsoft's 
clusters have runtimes $2\times$ larger than a lower bound. 
%$25$\% of DAGs are off by $4\times$. 
%Tetris and critical path scheduling are off by $x$\% and $y$\% respectively  for $50$\% of the DAGs.
}
\vskip .05in

With existing DAG schedulers, we observe that the worse schedules arise because: (a) long-running tasks  have no other work to overlap with them and (b) the tasks that are runnable do not pack well with each other. 
Based on these observations, {\name} incorporates one core intuition: to pack an entire DAG well, pay careful attention to tasks that can otherwise lead to a bad schedule. Building on this intuition, {\name} places such {\em troublesome} tasks first on a {\em virtual resource-time space} and then overlays the other tasks to fill any resultant holes in this space. Figure~\ref{fig:graphene_overview} shows an example. {\name} solves two key challenges in realizing this idea: (1) the best choice of troublesome tasks is intractable to compute and (2) since the above method binds tasks to space out-of-order it can reach {\em dead-ends}. For instance, if two tasks are bound first because they were considered troublesome, then there may not remain enough space to place tasks that lie between these two tasks on the DAG. Simply leaving some slack space is inefficient because it is apriori unclear how much should be set aside. {\name} employs a performant search procedure to combat the first challenge and a placement procedure that provably avoids dead-ends.

\cut{
 can lead to dead-ends.
 {\name} explores various options.  To scale, the search mimics dynamic programming. That is, it biases towards better subsets and prunes efficiently. Second,    {\name} divides the tasks into four subsets, as shown in Fig~\ref{fig:graphene_overview}, and uses provably feasible orders for placing these subsets. 
% That is, each order avoids dead-ends and all such orders are considered.
}
\cut{
\vskip .05in
{\name} decouples schedule construction from online packing and fairness guarantees.  The online component enforces the desired schedules of the various DAGs. In addition, {\name} offers a new packing heuristic that overbooks resources judiciously.  Furthermore, for a wide variety of desirable fairness schemes, {\name} improves performance while bounding the extent of unfairness.
}
\vskip .05in
To summarize, the key contributions of {\name} are: 
\begin{Itemize} 
\item A characterization of the DAGs seen in production at a large enterprise and an analysis of the performance of various DAG scheduling algorithms~(\xref{sec:packdeps}).
\item A novel DAG scheduler that combines multi-resource packing and dependency awareness~(\xref{sec:design}). 
%time while respecting dependencies~(\xref{sec:design}). 
\item An online scheduler that mimics the preferred schedules for all the jobs on the cluster and overbooks resources while ensuring bounded unfairness~(\xref{sec:runtime}).
\item A new lower bound on the completion time of a DAG of tasks~(\xref{sec:betterlb}).
\item An implementation that we intend to release as open source and contribute back to relevant Apache projects~(\xref{sec:system}) and extensive experiments on a $200$ server cluster~(\xref{sec:eval}). 
%We use a few tricks to meet the tight efficiency requirements needed to scale to clusters with thousands of machines and jobs~(\xref{sec:system}). 
{\name} improves completion time of half of the DAGs by $19-31$\%; the number varies across benchmarks.  The improvement for production DAGs is near the high end of the range~(half improve by at least $25$\%) because these DAGs have more user-defined code and diverse resource demands.
\end{Itemize}

\cut{That is, given a threshold $\kappa$, {\name} ensures that the gap from desired
fair share~(of cluster resources) never dips below $\kappa C$ where $C$ is cluster
capacity. We are not aware of any such scheduler for data-parallel clusters.

\vskip .05in
We develop a new lower bound on DAG completion time by 
using the specific structure of data-parallel DAGs. Unlike the case of an arbitrary DAG,
tasks in a stage are unordered with respect to each other and have similar durations, resource needs
and dependencies. This lower bound shows that {\name} is quite close to optimal.
That is, ${\name} \geq {\tt OPT} \geq {\tt NewLB}$ and {\name} is within $5$\% 
of ${\tt NewLB}$ for half of the considered DAGs. The optimal packing+dependencies solution is intractable to compute~\cite{MastrolilliS:2009}
and the available lower bounds are loose~\cite{StripPart,Mastrolilli:2008}. Thus, ${\tt NewLB}$
advances the state-of-art.
}

\eat{We use the specific structure of data-parallel DAGs
to develop a much tighter lower bound. That is, in contrast to random DAGs, all the tasks in a stage have similar dependencies,
durations and resource needs. 
The new lower bound is tighter by about $30$\% and 
Since, ${\name} \geq {\tt OPT} \geq {\tt Bound}$, {\name} is quite close to optimal.}



\cut{
\vskip .05in
{\name} combines multi-resource packing and dependency-awareness in the practical setting of a cluster scheduler. We offer an extensive review of related algorithmic work: {\em job shop} scheduling~\cite{Czumaj:2000,Goldberg:1997,Shmoys:1994},  {\em vector bin packing}~\cite{ChekuriK04,ImKMP15,AzarCG13} etc. Our summary is that (a) there are no useful results for the online case~\cite{AzarCG13}, (b) the algorithms make many simplifying assumptions that prevent using them in this more realistic setting~(e.g., only chains but not general DAGs~\cite{tpkelly1}, tasks have homogenous needs~\cite{tpkelly1},  at most two resources~\cite{StripPart}, one machine~\cite{StripPart}, zero cost pre-emption~\cite{} etc.), and (c) the best known offline algorithms are $\log ({\tt OPT})$ times ${\tt OPT}$ where ${\tt OPT}$ is the optimal makespan but even simple heuristics perform better in practice. {\name} offers a new heuristic that appears to have sizable practical gains for a variety of DAGs.
}

\vskip .05in
%\sriram{This is too far out.  Can we move this to the second para or so?}
Finally, while our work is discussed in the context of cluster scheduling thus far, similar packing+dependencies problems arise in other domains. 
We offer early results (\xref{subsec:other-domains}) from applying {\name} to schedule DAGs in distributed build systems~\cite{bazel,cloudmake} and request-response workflows~\cite{kwiken,c3}. 
\cut{
We also note that the network transfers in large queries~(e.g., multi-way joins) resemble coflows~\cite{varys,aalo} with dependencies. For example, word-count over a join of two datasets, is two shuffles, one per dataset, and a dependent shuffle to compute the wordcount. Scheduling such transfers well remains an open problem especially in a geo-distributed context~\cite{dje,iridium,geode}. We are working to extend {\name} to this problem.
}

\cut{two similar problems:  scheduling coflows~\cite{varys,aalo} with dependencies, a problem that arises when scheduling all of the network transfers in large queries~(e.g., multi-way joins), executing large queries in a geo-distributed context~\cite{iridium,geode,dje} scheduling problem~\cite{varys} is akin to multi-resource packing if you let each flow correspond to a task and each network link is a resource with different tasks(flows) requiring different amounts of each resource(link). Some recent work schedules independent coflows so as to lower the average completion time~\cite{aalo}. However, scheduling all of the network transfers that arise in a DAG is the problem of scheduling coflows with dependencies.  This problem remains open and  to coflows.}

\cut{
[Online] There are no known algorithms with bounded competitive ratio for the online case being consdered here~\cite{AzarCG13}. [Realistic Setting] Algorithmic work makes one or more of these simplifying assumptions: task's demands are  infinitely malleable, preempting tasks has negligible cost and cluster resources are in one big bag (and not divided) across many machines. [Practical gains] More importantly, the best-known offline results are logarithmic approximations~\cite{Shmoys:1994}, i.e., expected performance is $\log({\sf OPT}) \times {\sf OPT}$ where ${\sf OPT}$ is the optimal. Simple heuristics already perform better in practice. 
}
\cut{
The best-known 
algorithms obtain logarithmic approximation factors \cite{Shmoys:1994}. There are several impossibility results
for the online case~\cite{AzarCG13}. Further, our practical problem is a significant generalization 
due to a few reasons: 
%a task's resource needs will change if it loses locality, 
task's demands are not arbitrarily malleable, cluster resources are not one big bag 
leading to machine capacity being fragmented etc.
}

%  by (a) cutting
% a DAG such that there is no overlap in schedule between the parts which allows
% picking the best possible lower bound per part and (b) accounting for
% parallelism better. \fixme{say better} We apply this new bound to over $20$K DAGs
% seen in production at Bing. Our analysis shows that {\name} is within $5$\% of
% the optimal for over half these DAGs.

\cut{
\vskip .05in
We implemented the offline and online parts of {\name} by extending Tez~\cite{tez} and YARN~\cite{yarn}
respectively.
Several of our changes have been committed to open source.
Recurring jobs dominate in our clusters; up to $40$\% of the jobs 
run the same code over new data~\cite{rope}. We use their past job history
to estimate task durations and resource needs. For ad-hoc jobs, we use estimates based on 
the most similar previous job. Also, we measure task's resource usage and progress online.
%We will commit these changes to open source. Several parts have been checked-in already.
% The baseline
% schedulers in Yarn, capacity- and fair- schedulers, both greedily
% assign a task with good data locality from among the queue that is
% currently most under-served. With {\name}, the logic of both
% schedulers remains identical except for: (a) they pick a task per
% desired schedule for DAG, (b) they prefer jobs with less remaining
% work, (c) they overbook resources and (d) relax fairness for
% performance yet the extent of unfairness is bounded. 
Our experiments ran jobs from several benchmarks~(TPC-DS, TPC-H), and
production jobs at Microsoft on a $200$ server cluster.  Relative to
Tez, {\name} improves completion time of half of the DAGs by
$19-31$\%.  The improvements for production Microsoft DAGs are towards
the high end of the range~(half the DAGs speed up by $25$\% and a
quarter by $57$\%) because they have more user-defined code and
diverse resource demands.
%Relative to Tetris and Critical path, {\name} improves by $15-40$\%.
}
\cut{
\vskip .05in
To summarize, the key contributions of {\name} are: 
\begin{Itemize} 
\item A novel DAG scheduling algorithm that combines multi-resource packing and
dependency awareness. 
%time while respecting dependencies~(\xref{sec:design}). 
\item An efficient online scheduler that mimics the
desired order for all the jobs on the cluster, packs tasks, and overbooks fungible 
resources while ensuring bounded unfairness.
\item A new lower bound on the completion time of a DAG of tasks.
\item An implementation that has been partially contributed to relevant Apache 
projects, extensive experiments with Tez and Hive jobs on a cluster,  
and an analysis of the DAGs in Microsoft's clusters. 

%\item From analyzing $20$K production DAGs from
%Bing, the schedules constructed by {\name} are $25$\% faster for half the DAGs.
%A quarter improve by $57$\%. 
% \item By applying our new lower bound, we show that
% {\name}'s schedules are optimal for $40$\% of DAGs.
% Three quarters of the DAGs are within $13$\%.
\end{Itemize}
}
%why are we talking about this?
% The schedule construction algorithm, the online scheduler and the new lower bound are 
% described in~\xref{sec:design},~\xref{sec:runtime} and~\xref{sec:betterlb}.
% We begin with some background.

\eat{
Similar packing+dependencies scheduling problems arise elsewhere
too. We offer early results from applying {\name} to scheduling the
DAGs in distributed build systems~\cite{bazel,cloudmake} and
request-response workflows~\cite{kwiken}. \fixme{cya}
}




==> texfiles/introv4.tex <==
%!TEX root=../graphene.tex 
\section{Introduction} 
\label{sec:intro} 
DAGs (directed acyclic graphs) offer a powerful abstraction to
describe general scheduling problems. To name a few instances, the
data analytics jobs in Spark-SQL, Dryad and
Tez~\cite{tez,sparksql,dryad} as well as the network
transfers of multi-way joins which are coflows with
dependencies~\cite{varys,aalo}, all build around a DAG construct. The common abstraction
makes it possible to adapt previously-studied DAG scheduling
algorithms~\cite{tpkelly1,StripPart,Goldberg:1997} for the problems at
hand.  However, some of the key assumptions that underlie these scheduling  
algorithms (such as, homogeneity in the characteristics of DAG vertices) do not  always
hold in practice. Hence, the generated DAG schedules can be arbitrarily inefficient leading us
to explore novel approaches.
\cut{
% SK: while it is a bit over-bold, i prefer the above to the below; to be decided in next pass
The generated schedule represents an ordering of the DAG's
vertices while respecting the dependencies that are defined by
the DAG's edges.  We find that generating efficient schedules for
large/complex DAGs to be particularly challenging.
}

We illustrate the challenges in the context of DAGs that arise in
data-analytics clusters.  These clusters comprise of tens of thousands
of servers~\cite{bdas,bdas2} and run thousands of mission-critical
job DAGs each day. 
Furthermore, the more sophisticated programming models supported in these clusters~\cite{tez,sparksql,flumejava,dryad,scope-vldb12}  
lead to complex DAGs and vertices with diverse resource demands.  
Traces from a large cluster indicate that the median job has depth $7$, a thousand vertices~(or tasks)
and, the coefficient-of-variation~(stdev./avg.) in requirements for resources such as CPU, memory, disk   
and network is nearly $1$ across tasks. Our analysis of job completion times in this production cluster  
indicate that a speed-up of up to 50\% is possible for half the DAGs.   

A few reasons possibly account for the inefficiencies in scheduling
DAGs.  Production cluster
schedulers~\cite{yarn,apollo,omega} cope with many concurrent
jobs and short-lived tasks. Hence they have stringent time-budgets to
match pending tasks to available machines and consequently rely on
very simple heuristics.  On the other hand, the algorithmic problem of
scheduling even one DAG is
NP-hard~\cite{Mastrolilli:2008,MastrolilliS:2009}.  At a high
level, it requires compactly packing tasks with different
durations and demands for multiple resources, while respecting the inter-task
dependencies.  Consequently, prior work looks at several
special cases of the problem such as: assume jobs are known
apriori~\cite{Goldberg:1997}, ignore
dependencies~\cite{psv,reverse-fit,ImKMP15}, only chains but not
general DAGs~\cite{tpkelly1}, assume homogenous needs and use at most
two resources or run on only one machine~\cite{tpkelly1,StripPart}
%tasks use at-most two resources~\cite{StripPart}, 
%or run on only one machine~\cite{StripPart}
%, and can be pre-empted with zero cost~\cite{} 
etc. In fact the best known offline algorithm for a nearly realistic model 
has logarithmic guarantees~(i.e., no worse than $\log ({\tt OPT})$ times ${\tt OPT}$)
% where ${\tt OPT}$ is the optimal makespan 
but even simple heuristics such as critical path scheduling~\cite{coffman-graham,graham}
and Tetris~\cite{tetris} perform better in practice.

Given the high cost to build and maintain these large clusters, even
modest improvements in cluster utilization can significantly improve
ROI (return-on-investment).  Further, speeding up jobs can shorten the
lag between data collection and decisions (i.e., ``time to insight'')
which potentially increases revenue~\cite{velocityLatency}.

Motivated by these observations, we design and implement {\name}, a
new cluster scheduler for DAGs. Our goal is to retain the simplicity of today's production
schedulers in order to scale while more efficiently scheduling DAGs. We achieve this goal
as follows.

First, we decouple DAG schedule construction from the online time-stringent aspect of matching
tasks to machines. 
Hence, {\name} has two components.
An offline component that at job submission time or soon thereafter, builds a preferred schedule
for tasks in that job.
%The preferred schedule is an ordering over the tasks that leads to a compact global packing for the entire DAG. 
%{\name} reuses previously computed preferred schedules for recurring jobs~\cite{rope}. 
%An  online component {\em softly} enforces these preferred schedules across all of the jobs that are running concurrently
%in the cluster. Further, it does so while satisfying cluster sharing constraints such as fairness and locality~\cite{yarn,apollo,omega}.
An online component that {\em softly} enforces these preferred schedules across all of the jobs that are running concurrently
in the cluster.  The soft enforcement is needed to also satisfy unrelated cluster sharing constraints such as fairness and locality~\cite{yarn,apollo,omega}.

Second, we motivate the design of the offline component by observing that
the pathologically bad schedules in today's approaches mostly arise due to these reasons:
(a) long-running tasks have no other work to overlap
with them and (b) the tasks that are runnable do not pack well with
each other.  Our core idea, in response, is rather simple: identify the potentially {\em troublesome} tasks, such as those that run for a very long time
or are hard to pack, and place them first on a {\em virtual resource-time space}.
This space would have $d+1$ dimensions when tasks require $d$ resources; the last 
dimension being time. Our claim is that placing the troublesome tasks first
leads to a good schedule since the remaining
tasks can be placed into resultant holes in this space. Further, {\name}
solves two key challenges in realizing this idea: (1) the best choice
of troublesome tasks is intractable to compute and (2) {\em dead-ends}
may arise because tasks are placed out-of-order~(e.g., troublesome go first)
and it is apriori unclear how much slack space shoud be set aside.
{\name} employs a performant search procedure to address the first challenge
and has a placement procedure that provably avoids dead-ends for the second challenge.
\autoref{fig:graphene_overview} shows an example. 
\begin{figure}[t!]
\centering
\includegraphics[width=3in]{figures/graphene_overview.png}
\ncaption{Shows steps taken by {\name} from a DAG on the left to its schedule on the
right. Troublesome tasks~${\tt T}$~(in red) are placed
first. The rest of the subsets~(parents~${\tt P}$, children~${\tt C}$ and other~${\tt O}$) 
are placed {\em on top} of ${\tt T}$ in a careful order that ensures compactness and respects
dependencies.\label{fig:graphene_overview}}
\end{figure}


Third, the online component matches tasks to machines at scale by
using a simple heuristic that reconciles multiple, potentially
discordant, objectives. For example, a fairness scheme such as DRF may
require a certain queue to get resources next, multi-resource packing
which we use to improve cluster utilization may pick a different task
to schedule than DRF, and the schedules constructed above may pick yet
a third task. The heuristic combines these various objectives into one
real-valued score thereby violating any one objective only if enough
other objectives counterweigh it.  Further, we do the above while
limiting the maximum amount of unfairness to an operator configured
threshold; we can do this for many models of fairness~\cite{yarnFS,kellyPF,drf}
and doing so helps ensure predictable performance.

\cut{
\vskip .05in
If there was only one resource and no dependencies, any work-conserving scheduler would do reasonably.  Because state-of-the-art proposals do either multi-resource packing or dependency-aware scheduling, they  fail to achieve good performance.
%
%By doing only one of the two-- multi-resource packing or dependency-aware scheduling--state-of-the-art proposals fall short.
For instance, packers~\cite{tetris,vector} greedily pick the best-packed task and ignore dependencies.  However, the best-packed task need not have the longest critical path. And, local greedy choices are unlikely to lead to a good {\em global} packing for the entire DAG. In fact, we show that {\em any scheduler} that ignores dependencies will be $\Omega(d)\times$ optimal when tasks need $d$ resources.\footnote{ 
In practice, there are at least four resources~(cores, memory, network and disk), i.e., $d\geq 4$.}
%Tetris is at least $(d+1)\times$ away. 
On the other hand, dependency-aware schedulers~\cite{coffman-graham,graham} assume tasks have homogeneous demands. We show that: when tasks have varying demands, by not packing, these algorithms are up to $n\times$ optimal,  where $n$ is the number of tasks in the DAG. Typically, $n\geq 100$~\cite{rope,mantri}.

Finally, production cluster schedulers~\cite{tez,yarn} schedule based on exogenous factors such as 
locality and fairness. Our analysis shows that $50$\% of the DAGs in Microsoft's 
clusters have runtimes $2\times$ larger than a lower bound. 
%$25$\% of DAGs are off by $4\times$. 
%Tetris and critical path scheduling are off by $x$\% and $y$\% respectively  for $50$\% of the DAGs.
}
\vskip .05in



\cut{
 can lead to dead-ends.
 {\name} explores various options.  To scale, the search mimics dynamic programming. That is, it biases towards better subsets and prunes efficiently. Second,    {\name} divides the tasks into four subsets, as shown in Fig~\ref{fig:graphene_overview}, and uses provably feasible orders for placing these subsets. 
% That is, each order avoids dead-ends and all such orders are considered.
}
\cut{
\vskip .05in
{\name} decouples schedule construction from online packing and fairness guarantees.  The online component enforces the desired schedules of the various DAGs. In addition, {\name} offers a new packing heuristic that overbooks resources judiciously.  Furthermore, for a wide variety of desirable fairness schemes, {\name} improves performance while bounding the extent of unfairness.
}
\vskip .05in 
% line left blank
To summarize, we make theoretical as well as practical
contributions in this work.  Our key contributions are:
\begin{Itemize} 
\item A characterization of the DAGs seen in production at a large
  enterprise and an analysis of the performance of various DAG
  scheduling algorithms~(\xref{sec:packdeps}).
\item A novel DAG scheduler that combines multi-resource packing and
  dependency awareness~(\xref{sec:design}).
%time while respecting dependencies~(\xref{sec:design}). 
\item An online scheduler that mimics the preferred schedules for all
  the jobs on the cluster while bounding unfairness~(\xref{sec:runtime}).
\item A new lower bound on the completion time of a DAG~(\xref{sec:betterlb}). Using this we show that the DAG schedules built by {\name}
  are within $1.04$ times ${\tt OPT}$ for half of the production DAGs; three quarters are within $1.13$ times
  and the worst is $1.75$ times ${\tt OPT}$.
\item An implementation that we intend to release as open source~(\xref{sec:system}),
  extensive experiments on a $200$ server cluster
  and simulations on $20,000$ DAGs from production traces~(\xref{sec:eval}).
%We use a few tricks to meet the tight efficiency requirements needed to scale to clusters with thousands of machines and jobs~(\xref{sec:system}). 
{\name} improves completion time of half of the DAGs by $19-31$\%; the
number varies across benchmarks.  The improvement for production DAGs
is near the high end of the range~(half improve by at least $25$\%)
because these DAGs have more user-defined code and diverse resource
demands.
\end{Itemize}

Lastly, while our work is presented in the context of cluster
scheduling, as noted above, similar packing+dependencies problems arise in
other domains.  We offer early results in~\autoref{subsec:other-domains}
from applying {\name} to scheduling DAGs arising in distributed build
systems~\cite{bazel,cloudmake} and in request-response
workflows~\cite{kwiken,c3}.

\cut{That is, given a threshold $\kappa$, {\name} ensures that the gap
  from desired fair share~(of cluster resources) never dips below
  $\kappa C$ where $C$ is cluster capacity. We are not aware of any
  such scheduler for data-parallel clusters.

\vskip .05in 
We develop a new lower bound on DAG completion time by
using the specific structure of data-parallel DAGs. Unlike the case of
an arbitrary DAG, tasks in a stage are unordered with respect to each
other and have similar durations, resource needs and
dependencies. This lower bound shows that {\name} is quite close to
optimal.  That is, ${\name} \geq {\tt OPT} \geq {\tt NewLB}$ and
{\name} is within $5$\% of ${\tt NewLB}$ for half of the considered
DAGs. The optimal packing+dependencies solution is intractable to
compute~\cite{MastrolilliS:2009} and the available lower bounds are
loose~\cite{StripPart,Mastrolilli:2008}. Thus, ${\tt NewLB}$ advances
the state-of-art.  }



\cut{
\vskip .05in
{\name} combines multi-resource packing and dependency-awareness in the practical setting of a cluster scheduler. We offer an extensive review of related algorithmic work: {\em job shop} scheduling~\cite{Czumaj:2000,Goldberg:1997,Shmoys:1994},  {\em vector bin packing}~\cite{ChekuriK04,ImKMP15,AzarCG13} etc. Our summary is that (a) there are no useful results for the online case~\cite{AzarCG13}, (b) the algorithms make many simplifying assumptions that prevent using them in this more realistic setting~(e.g., only chains but not general DAGs~\cite{tpkelly1}, tasks have homogenous needs~\cite{tpkelly1},  at most two resources~\cite{StripPart}, one machine~\cite{StripPart}, zero cost pre-emption~\cite{} etc.), and (c) the best known offline algorithms are $\log ({\tt OPT})$ times ${\tt OPT}$ where ${\tt OPT}$ is the optimal makespan but even simple heuristics perform better in practice. {\name} offers a new heuristic that appears to have sizable practical gains for a variety of DAGs.
}











==> texfiles/maindeltas.tex <==
1) No existing system has optimized over whole job DAG.  There are theoretical works that do, but they are unlikely to work in practice since they abstract away many practical issues. (packing/ online (dynamic)).  Cost-based optimization; how to move operators around etc.; not once you have a DAG how to schedule that DAG; taking into account cluster conditions.

2) Scheme (+DAG, +packing, +online)

3) Measurement study of real DAGs <- first to look at all aspects of the DAG that are relevant for scheduling.

4) +completion time; + fairness.


We looked at packing in Tetris; but just doing that on a DAG is screwy. Only a subset of all tasks are available to run at any time; myopically optimizing the packing on them is not too good; dynamic aspect, how currently runnable tasks are scheduled influences which become ready later; may be better packable later than before; so have to worry about DAG structure; amount of resources matter.

==> texfiles/measurements.tex <==
\section{Analysis of Production DAGs}

In this section, we present characteristics of job DAGs in a
production Cosmos~\cite{cosmos} cluster at Microsoft. Although out
study is limited in scope, we believe it is the first measurement
study of production job DAGs from a large analytics cluster. Our
objective in doing so is not only to advance our understanding of
analytics jobs beyond the narrow Map-Reduce model but also to motivate
our solution in {\name}.

The Cosmos~\cite{cosmos} production cluster consists of many thousands
of machines executing $\mathcal{O}\left(10000\right)$ jobs every
day. The job scripts (submitted in Scope~\cite{scope}) are converted
to a DAG of stages where each stage executes many parallel tasks. The
machines in the cluster are well-provisioned with CPU cores ($16$),
memory ($32$GB), disk storage and network links ($10$Gbps). The tasks
in the {\em input} stage read data from the underlying distributed
file system and pass their outputs to downstream {\em intermediate}
tasks.




\subsubsection{Stage Characteristics}

\begin{figure}[t!]
\centering
\subfigure[Stage Properties]{\includegraphics[width=1.5in]{figures/Measurements/stages.pdf}\label{fig:stages}}
\subfigure[As $\%$ of Stages]{\includegraphics[width=1.5in]{figures/Measurements/stages-percent.pdf}\label{fig:stages-percent}}
\caption{Stage Characteristics. We plot the CDF of the number of stages in a job, in its critical path, and that simultaneously execute.} \label{fig:stage}
\end{figure}

\noindent{\bf Depth and Width:} Figure~\ref{fig:stages} plots the distribution of the number of stages across DAGs. While the median number of stages is $9$, a few jobs have over $100$ stages. An important characteristic in scheduling such jobs is the critical path, as explained earlier. As Figure~\ref{fig:stages} shows, the number of stages in the critical path varies considerably. In fact, they can constitute $40\%$ of all the stages in the job's DAG at median (Figure~\ref{fig:stages-percent}).

In fact, while some jobs have long critical paths, many others are
``wide''. Figure~\ref{fig:stages} and \ref{fig:stages-percent} also
measure the {\em maximum} number of stages whose tasks execute in the
job's DAG at any given time. The maximum width can be nearly half the
total number of stages in the job, at median. We also that there is
only moderate correlation in a DAG between the length of its critical
path and maximum width (correlation coefficient of $0.41$; the
coefficient is $0.33$ when viewed as a fraction of total
stages).

Overall, these results highlight the importance of developing general
scheduling techniques that focus on richer DAGs (i.e., deep and/or
wide) than the two-staged MapReduce jobs.
%, by simultaneously dealing with jobs that are both long as well as wide (in number of stages).
%
%\begin{figure}[t!]
%\centering
%\includegraphics[width=3.2in,height=1.2in]{figures/Measurements/comm.pdf}
%\caption{Breakdown by Communication Pattern. \textcolor{Red}{Revisit}} \label{fig:comm}
%\end{figure}

\noindent{\bf Communication Patterns:} Analytics jobs have varied
communication patterns among their stages. Stages that perform a
simple transformation of data usually have a ``one-to-one''
relationship with their previous stage. Some stages perform partial
aggregation of data from the previous stage, leading to a
``many-to-one'' pattern~\cite{sosp09}. Joining of two tables of data
also results in ``many-to-one'' communication. Reduction operations
(e.g., group-by, count) result in ``all-to-all''
communication. One-to-one, many-to-one and all-to-all communication
patterns occur $31\%$, $46\%$ and $23\%$, respectively, in the
traces. This implies that a DAG scheduler should deal with a variety
of communication patterns, since each of it poses different resource
requirements on the remote machines from which data is read.

\eat{
We break down stages by their communication pattern and share of the various resources used by them. The three communication patterns are equally represented in occurrence. Phases with one-to-one communication dominate the data read and CPU/memory consumed because they include the ``extract'' stage that reads the input data of the job and contains a large number of tasks; they contribute less than a quarter to data that flows over the network. Surprisingly, the ``all-to-all'' stages account for a small fraction of all the resources, including the network. Stages with many-to-one communication account for a higher fraction. As mentioned above, these are stages that perform table joins as well as partial aggregation (before the all-to-all full aggregates). This not only indicates effective data reduction due to partial aggregates, \aditya{is this something graphene needs to track for network resource requirement?} but also the need to optimize the network for many-to-one communication instead of the traditional focus on all-to-all ``shuffle'' communication. \aditya{hard to draw a connection to graphene. does this guide overbooking? i don't think so..}
}

\begin{figure}[t!]
\centering
\includegraphics[width=3.2in,height=1.2in]{figures/Measurements/potential.pdf}
\caption{Potential Analysis. We understand the impact of critical path
  scheduling and resource availability on DAG scheduling. There is a
  potential for $45\%$ improvement at median using a technique that
  combines critical path and resource
  availabilities.} \label{fig:potential}
\end{figure}

\subsubsection{Scheduling Constraint}

As described in \xref{subsec:problem}, the two axes of importance in
DAG scheduling are the critical path and the resource consumption of
the stages. We now analyze the importance of each of these factors on
scheduling. We use a ``what-if'' analysis to analyze these two axes
one at a time: loosen the restriction on the other axis such that
only one axis matters.

%\aditya{changed dimension to axis as dimension could be confused with resource dimension}

Figure~\ref{fig:potential} plots the difference in job duration
between the trace and as obtained from its critical path analysis
(``critical path based gap''). The critical path analysis assumes
enough resources for all the {\em simultaneously runnable} tasks of a
stage to execute. Thus, only its critical path matters. Every stage's
duration is just the duration of its longest task. We see a nearly
uniform curve with substantial difference between the durations in the
traces and those achievable by its critical path; median and
third-quartile differences are $45\%$ and $66\%$,
respectively.\footnote{The calculation, however, omits {\em
    pipelining} between stages, and is thus on the conservative side.}

We next analyze the impact of restricting the resources available to
the job (to that in the original trace). To do so, we loosen the DAG
requirement by having no dependencies between the tasks of a job,
essentially treating all the tasks of a job as one big bag. In this
model, the number of simultaneous tasks of a job are restricted by the
available resources (in CPU, memory, disk and network bandwidths), and
thus will run over multiple ``waves''. We compare the job duration
obtained thus to the actual duration in the trace. As
Figure~\ref{fig:potential} shows, resource limitation appear to be
playing relatively less of a role than the critical path of the DAG
(``resource based gap'') in Cosmos' production scheduler. The gap is
higher than that obtained by the earlier critical path
analysis, beyond the tenth percentile, implying that the Cosmos
scheduler generally does a better job of meeting resource requirements
than it does of optimizing critical path performance; retaining dependency restrictions mattered more than retaining resource restrictions. Nevertheless, the gap is still significant in
absolute terms indicating there is room for improvement there as well.

%\noindent{\bf Potential:} Given the above analysis and importance of
%both critical path analyses and resource availability, what is the
%upper bound for improving job completion time in the Cosmos traces? We
%measure it calculating the maximum of the achievable job durations
%when restricted using the critical path (critical path based gap) and
%resources (resource based gap). The ``potential'' curve captures this
%as a CDF across jobs in Figure~\ref{fig:potential}. Often, critical
%path restrictions turn out to be more significant, with the potential
%curve overlapping with the critical path gap for the most part. The
%potential improvement in job completion time is $45\%$ at median, all
%the way up to $>90\%$. Since critical path here assumes infinite
%resources, gains achieved in practice from careful scheduling of
%DAGs may be much more limited.

%\noindent{\bf No correlation between DAG properties and gap to
%  critical path duration}. We observe little correlation between the
%gap to the critical path duration and notable DAG properties. The gap
%exhibits a correlation coefficient of $0.15$, $0.12$, $-0.35$, $0.1$
%and $-0.3$ with the number of stages, width, width as a fraction of
%the number of stages, critical path length, and the length as a
%fraction of the number of stages, respectively.

We next present a technique that combines both these aspects in its scheduling.

\subsubsection{Impact of overallocation}

The Cosmos production scheduled~\cite{cosmosscheduler} does not use a fixed number of compute slots per machine; instead, it starts new tasks when resources are available. This leads to potential overallocation of resources, increasing the latencies of running tasks. In this section, we quantify the impact of resource overallocation on node latency by correlating resource utilization with relative slowdown of tasks in the same stage.

Methodology: for each stage in a job, compute the median node latency and select nodes with latencies that differ from the median by at most 50\%. We only use stages with median latency of at least 10 seconds to reduce noise (we only have resource measurements with granularity of 2 minutes). For each task, we compute its \emph{slowdown} as $(L-A)/A$, where $L$ is the task latency and $A$ is the average latency of tasks in this stage. For each task we also compute the average utilization of the various resources during the task execution. 

Figure~\ref{fig:overallocation} shows the impact of overallocation of the major resources on task slowdown. X-axes show the utilization of each resource (except that figure~\ref{fig:over_mem} shows ``free memory''); see units in the caption. We quantize resource utilization and for each bucket, we compute the average, median and 75th percentile of task slowdown (blue, gray, and yellow lines). The orange line shows the number of observed tasks at a particular utilization. 

Observations: clear impact of resource overallocation for CPU (up to 60\% slowdown), for memory (up to 1.2x slowdown) but don't have much data, and maybe for disk reads (up to 0.5x slowdown). Notice that steep increase in slowdown for high CPU utilization.

\emph{How to present this?} remove the ``count'' line and only show values where we have enough support; eg, only where we have at least 100 nodes in a bucket. Do we discuss the dip at low CPU utilization? we don't have a good answer what's going on there. just show the average line for CPU, memory and disk read?

\begin{figure}[!]
\centering
\subfigure[CPU]{\includegraphics[trim=0 75 0 90, clip, width=2.5in]{figures/Measurements/over_cpu.pdf}\label{fig:over_cpu}}
\subfigure[memory (unit: 1GB)]{\includegraphics[trim=0 75 0 90, clip, width=2.5in]{figures/Measurements/over_mem.pdf}\label{fig:over_mem}}
\subfigure[NIC (unit: 10MB/sec)]{\includegraphics[trim=0 75 0 90, clip, width=2.5in]{figures/Measurements/over_net.pdf}\label{fig:over_net}}
\subfigure[disk read (unit: 10MB/sec)]{\includegraphics[trim=0 75 0 90, clip, width=2.5in]{figures/Measurements/over_diskread.pdf}\label{fig:over_diskread}}
\subfigure[disk write (unit: 10MB/sec)]{\includegraphics[trim=0 75 0 90, clip, width=2.5in]{figures/Measurements/over_diskwrite.pdf}\label{fig:over_diskwrite}}
\caption{Impact of resource overallocation.} \label{fig:overallocation}
\end{figure}


\eat{
Actual job runtime vs. Critical path length.

Compute area of DAG to estimate how many different resources are substantial/ which ones are they?

How constrained are the resources?  Size of cluster vs. max potential parallelism in DAG vs. actual parallelism achieved at runtime.

How many DAGs are running at any one time?  Some measure of how different they may be/ how packable they may be.

How estimatable are resources? Recurring jobs? Within a stage? In Tetris, we just did a brute comparison, would fitting a regex to input size be better?

Need for dynamism: a slightly subtle point, we will make, is that it is better to schedule the lists dynamically. it would be good to argue that this is because of (runtime) outliers, i.e., tasks taking longer than one would expect. Any measures of that will help.

measurements vs. sim: Mimicing critical path scheduling/ packability may be best done in simulator. Looking for hard measurement data here.

Graph note: CDFs for most measures are okay; perhaps illustrative examples.  When doing a CDF either do per job or weigh jobs on their contribution to cluster-hours.

Minor:
Depth (\# of stages).
Barriers (input-output dependencies).
Some stages are much shorter (duration) or wider (resource usage) than others.
}


==> texfiles/old/a.tex <==
%!TEX root=../paper.tex
\section{Introduction}

Tasks have diverse resource demands, along CPU, memory, network and disk bandwidth. Packing tasks of a job well, i.e., placing them on machines and times such that more tasks run simultaneously, can speed-up a job substantially~\cite{tetris}. Further, a scheduler that packs well allows a cluster to run more jobs in the same amount of time (or lower makespan of the set of jobs).

A key obstacle in reaching this goal is the dependencies between tasks. Input-output dependencies among tasks within a job require that a task begin only when all (or a large fraction) of its upstream tasks finish.  Typically, a task depends on many tasks.  Map-reduce\cite{XXX} jobs have a dependency graphs with depth $2$; however, more general DAGs that are used by Dryad, Tezz, Hive, SCOPE and Shark can have depth up to XXX. Similar dependencies also exist across jobs, in the context of pipelines where one or more downstream jobs process the output of a job~\cite{jockey}.

Dependencies complicate packing since at any time only a subset of all tasks are available to schedule.
This subset may or may not contain tasks that pack well together.
There is a dynamic aspect as well since a scheduling decision now impacts which tasks will be available for packing later.

Intuitively, packing DAGs is hard due to a tension between respecting critical path vs. respecting packing efficiency.  Both are useful. But, the order of scheduling tasks advocated by either approach varies substantially and choosing either order can increase job latency. For e.g., strict adherence to critical path may lead to bad fits and resource fragmentation. Strict adherence to packing efficiency can delay tasks on the critical path. Critical path scheduling is more problematic when the cluster is busy; since any resource fragmentation will lower throughput. Packing is problematic when the cluster is idle; since any delay in scheduling the next task on the critical path will impact job latency. Hence, resolving this tension requires a dynamic solution that is aware of resource availability and online arrivals of jobs.

Scheduling tasks with dependencies on multiple processors is a known NP-hard problem~\cite{XXX}. Critical path scheduling, i.e., scheduling tasks in descending order of their longest (downstream) path to a leaf task, is roughly $2$-approx~\cite{graham_scheduling} under some ideal conditions. However, critical path scheduling does not capture task resource requirements. We show by counter-example with a single resource that critical path scheduling can take up to $n \times$ longer than optimal, where $n$ is the number of stages in the DAG. Some recent work achieves a $\log n$-approximation for the case when tasks require only one resource~\cite{XXX}.  Extending the theoretical guarantee to the case of multiple resources is challenging because they rely on specialized packing algorithms~\cite{A2} that cannot pack vectors of resources~\cite{XXX}\footnote{Vector packing differs from packing {\it space}. In a 2d euclidean space for e.g., the following allocation is allowed \includegraphics[width=.1in]{figures/rectVvector_1.pdf}, where the black and red squares are different tasks. If the x-axes was cores and the y-axes memory, such an allocation is physically impossible. Vector packing requires allocations to not overlap on any dimension, as shown here  \includegraphics[width=.1in]{figures/rectVvector_2.pdf}.}.

{\name}



==> texfiles/old/background-old.tex <==
%!TEX root=../graphene.tex
\section{Background: Scheduling DAGs}
\label{sec:background}

Jobs in today's data-parallel clusters are specified as directed acyclic graphs~(DAGs), in which, (1) nodes represent one or moretasks that can run in parallel and (2) edges encode data
dependencies. A DAG's execution proceeds by scheduling {\em
runnable} tasks on the available processors. Each task has some
resource demands and is runnable when all data dependencies are
met -- i.e., it has either no input edges or all its upstream
tasks have finished.

\subsection{Problem definition}
\label{subsec:perdagproblem}
Each job is represented as a directed acyclic graph $\mathcal{G}= \{V, E\}.$ Each node in $V$ is a task. Tasks have demands
along four resource dimensions~(cores, memory, disk and network
bandwidth) represented in vector form as $\mathbf{r}$. Depending on placement, tasks may need resources at more than one
machine~(eg input is remote) or along network paths. Tasks may
be allocated a resource vector $\mathbf{a}$ that is less than
their (peak) demands, i.e. $\mathbf{a} \leq \mathbf{r}$. Task
duration $d$ is a convex function of resource allocation
$\mathbf{a}$ defined for $\mathbf{a} \in [0, \mathbf{r}]$. That
is, allocating less than peak resources causes the task to take
longer to run. This function need not be continuous or
differentiable since underallocating different kinds of
resources can have very different impact on the task.

The cluster is a collection of machines, with resource capacity
vector~$\mathbf{c}$ organized per some network topology. We
assume that the core is congestion-free. That is, the only
network bottlenecks are at the source or destination machines.
This is a typical scenario today due to the adoption of full
bisection topologies~\cite{vl2,fattree}.

The goal of the cluster scheduler is to (a) divide cluster
resources among groups of jobs per some requirement~(eg DRF or
Slot-fairness), (b) have high goodput~(measured in terms of
amount of useful work done) and (c) reduce average job
completion time. The latter two requirements are directly
impacted by packing~(avoids resource fragmentation) and
scheduling~(avoid lulls on the critical path).
\fixme{online; some recurring jobs so can plan}
\fixme{polish, prune un-needed concepts}

\begin{figure}
\begin{subfigure}[b]{0.5\textwidth}
\centering
\includegraphics[width=1.8in]{figures/g_3xoff.png}
\end{subfigure}
%
\begin{subfigure}[b]{.9\textwidth}
\begin{scriptsize}
\begin{tabular}{l|l|c|c}
{\bf Technique} & {\bf Execution Order} & {\bf Runtime} & {\bf
Worst-case}\\\hline
{\bf OPT} & {$t_1\rightarrow t_4 \rightarrow \{t_0, t_2, t_5\}
\rightarrow t_3$} & {$T$} & {$-$}\\
{\bf Crit. Path} & {$t_0 \rightarrow t_4 \rightarrow t_5
\rightarrow t_1 \rightarrow t_2\rightarrow t_3$} & {$3T$} &
{$O(n)\times$OPT}\\
{\bf Tetris} & {$t_0\rightarrow t_1\rightarrow t_2\rightarrow
t_4\rightarrow t_5\rightarrow t_3$} & {$3T$} & {$O(d)\times$
OPT}\\
\hline
\end{tabular}
\end{scriptsize}
\end{subfigure}
%\ncaption{\label{fig:eg1}}
\caption{DAG execution schedules derived used a few
representative algorithms. Since these algorithms do not
simultaneously pack along both the spatial and temporal
dimensions, their schedules are much higher than optimal (OPT).}\label{fig:eg1}
\end{figure}


\cut{
is started by scheduling nodes with no input edge are
schedulable for
execution (i.e., {\em runnable}) at any time. Whenever an
upstream stage completes
execution, it generates data for one or more stages in the
dependent downstream nodes;
a downstream stage becomes runnable when all the inputs for that stage are generated.
The job execution is complete when
all of the DAG's stages have completed execution.
}

\cut{In this seciton, we examine some salient aspects of the
DAGs generated by Tezz
and the Cosmos system used in Bing. We also describe the
state-of-the-art in DAG scheduling across a wide variety of
frameworks.}

\subsection{An example}
\label{subsec:problem}
Consider the DAG shown in Figure~\ref{fig:eg1}, where edges
encode dependencies among nodes. The labels for every node
represent the task duration~(top) and the demands for two
resources~(bottom). Assume that the total resource available is
$1r$ and let $\varepsilon$ represents a small value. \robert{the following sentences are too abstract. Either cut and just say:
The optimal schedule is shown below the figure. Or need a bit
more explanation if we go in details.} At time $0$, tasks $t_0,
t_1, t_4$ are schedulable. The optimal schedule is shown below
the figure. It overlaps the execution of all the long-running
tasks $t_0, t_2, t_5$.

Today's big data schedulers~\cite{tez,hive,hadoop} will execute
the task that finds a suitable placement first. Across jobs,
fairness is also often used. Both these criteria are exogenous
from the perspective of a DAG. \robert{I don't really understand the connection between the following sentences and the before
ones. Do you want to argue that existing techniques do not
perform well ?}We perform Monte Carlo simulations that (a) pick
the next task to run at random from among those that are
schedulable and (b) are work-conserving. The average runtime is
$x$ with an stdev of $x$.

Critical Path scheduling (CPSched) picks tasks along the
critical path (CP). The CP for a task is the longest path from
the task to the job output. The figure also shows the task
execution order with CPSched.~\footnote{CP of $t_4$ is $T$ and
that of $t_1$ is $(1-2\varepsilon)T$. The demands of tasks $t_0,t_1,t_4$ are large enough that they cannot run simultaneously.}CPSched ignores the resources needed by tasks and does not pack.In the particular case of this example, CPSched performs poorly
because scheduling tasks that are not on the critical path~(such as $t_1, t_4$) first would reduce overall resource
fragmentation.

A recent proposal, Tetris~\cite{tetris}, explicitly packs along
multiple resource dimensions. Tetris greedily picks the task
that fits within available resources and has the highest value
of the dot product between task demand vector and the available
resource vector. The figure also shows the task execution order
with Tetris.~\footnote{The L1 norm of $t_0, t_2$ is $0.9$
whereas that of $t_1$ is $0.8$ and $t_4$ is $0.7.$ When no other task is running, the dot product computed by Tetris equals the
L1 norm of resource demand.} Tetris does not account for
dependencies. Its packing heuristic only considers the tasks
that are currently schedulable. In the particular case of the
above example, Tetris performs poorly because it will not adopt
an inferior packing option first~(such as running $t_1, t_4$
instead of $t_0$) even though doing so, it would lead to a much
better packing of the downstream tasks.

More generally, we can show that critical path scheduling can be $O(n)\times OPT$ for a DAG with $n$ nodes.
Tetris has slightly better worst-case behavior. It can be
$(d+1)\times OPT$ when tasks require $d$ kinds of resources.
The proof is in the Appendix.
In practical clusters, $d$ is at least $4$~(cores, memory,
network, disk), and often larger when tasks require resources
at other servers~(that have task input for example) or along
network hops. The DAG size~($n$) is typically much larger
whereas jobs can have as many as $10^5$ tasks. We believe that
other scheduling algorithms such as breadth-first
traversal~\cite{}, coffman-graph~\cite{} have similar worst case behavior when packing+scheduling DAGs of tasks with multiple
resource dimensions.

Prior algorithmic work considers several simpler special cases
of the packing+scheduling problem.
In scheduling, for the special case of a {\em tree} wherein all
tasks have the {\em same demand} for a {\em single resource},
$2$-approx solutions are
available~\cite{criticalpath,coffman-graham}. In our context,
these solutions become $n$-approx.
As for packing, several approaches consider tasks with arbitrary demands for multiple resources~\cite{onlineVectorPacking}.
Tetris~\cite{tetris} is the state-of-the-art since it also
allows for tasks' demands changing with placement in an online
manner. We already saw that Tetris is $d+1$-approx when tasks
have dependencies.
In packing+scheduling, for the special case of a single
resource, the best known result offers a $\log n$
approximation~\cite{stripPartitioning}. Note that $\log n$ is a
weak bound since DAGs can have many nodes. In practice, we find
this algorithm to perform worse than the above simpler
solutions.
Also, we are unaware of any work that considers DAGs of tasks
that require arbitrary amounts of multiple resources and can
tolerate malleable allocations. {\name} is able to deal with all the afore mentioned limitations but also further considers the
case when the cluster is shared by different jobs.
\fixme{be more precise; what are we missing?}

\cut{
A practical issue with CP is that it is non-trivial to reliably
estimate task durations. More fundamentally, however, since CP
ignores
resource usage, it does an arbitrary job with packing leading
toresource fragmentation and delays. We illustrate the issues
using the
DAG in Fig.~\ref{fig:p_eg2}. Critical path for tasks $0, 1$ is
$4t,
8t$ respectively. The schedules shown in that figure illustrate
that
ignoring the critical path and scheduling task $0$ first leads
to an
almost 50\% speed-up. This is because it enables task $2$ and
task $3$
to run alongside task $1$, and thereby avoids resource
fragmentation.
In fact, the performance loss (such as, loss in throughput, job
slowdown, etc.) induced by focusing strictly on critical path
based-scheduling can be arbitrarily worse. To illustrate,
consider the
(slightly larger) DAG in Fig.~\ref{fig:p_eg3}, CP would schedule tasks
left-to-right; an optimal packer could instead schedule the
tasks with
$\{\epsilon t, .9r\}$ first such that all the tasks with
non-trivial
durations run simultaneously. The end-result is that, due to
resource
fragmentation, CP-based scheduling is over $4\times$ slower
whencompared to an optimal packing based scheduler.
}



\cut{
the amount of
cluster resources available impacts the choice of schedulers.
The more
constrained the resources, the larger the incentive to search
for a
good packing in the DAG. Moreover, the trade-off also depends on the
nature of DAG since the set of runnable tasks in the future
depends on
which tasks were chosen by prior scheduling decisions, and a
poor
choice can have long impact on the overall DAG execution time.
}

\cut{
We take care to point out three aspects. First, the simple
example above can be generalized to the case where each node in
the graph corresponds to a {\it stage} (such as map or reduce)
consisting of many tasks. Second, suppose task $0$ does get a
suitable placement first, there is an oppurtunity cost for the
job in ignoring this and continuing to wait for a suitable
placement for task $1$. Indeed, this is a crucial point, and one that we will build on in {\name}. Finally, if there were no
resource constraints, that is cluster capacity is $\infty$, then all of the schedules have the same runtime.
}

\cut{
Again, we note a couple broader points. First, the cluster often has many tasks and DAGs to run simultaneously. So, the resource
fragmentation in the above example can impact cluster goodput
but the impact on DAG runtime is often much larger. Second, the
performance penalty for critical path scheduling due to its
inability to pack can be arbitrarily worse. }

\cut{ Recently, some packing schedulers have been
  proposed~\cite{XXX}. They explicitly lower resource
fragmentation. Because they do not consider task dependencies,
they
are more appropriate for DAGs of small depth (e.g., one map
stage
followed by one reduce). In particular, on the above examples,
Tetris~\cite{tetris} takes $22t, 8t, 8t$ to execute
  Figures~\ref{fig:p_eg1}, ~\ref{fig:p_eg2}, ~\ref{fig:p_eg3}
respectively. These results are mixed. Optimal finishes in $15t,8t,
8t$. Because it packs, Tetris can improve upon CP. But because
it
ignores the DAG, it can do worse as well. We emphasize that
Tetris
does not look to enhance packability across nodes in the DAG;
so,
even in cases where critical path length is not a deciding
factor,
  Tetris can do (much) worse than the optimal packer.  }

\cut{
{\bf think: } What happens with multiple resource dimensions?
Greater depth of DAG?
}





\subsection{Analyzing DAGs in Production}
To ground the discussion, we examine the jobs from a production
cluster of tens of thousands of servers. Users write jobs in a
high level language~\cite{SCOPE} which is then compiled to a DAG by a query optimizer. We also analyzed the jobs from several
internal clusters that ran Hive/Hadoop jobs as well as some
high-performance computing~(HPC) workload~\cite{condor}. To get
a better sense of how complex are the generated DAGs, we
performed a simple analytical study.

The first question to ask is how deep are the DAGs ? By depth,
we refer to the number of tasks on the critical path. A
map-reduce job has depth $2$; the deeper a DAG, at first blush,
the more carefully one has to consider dependencies. We find
that the median (75th, 95th percentile) DAG has depth X1 (X2,
X3).

\begin{table}
\centering
{\small
\begin{tabular}{p{.68in}||c|c|c|c|c|c|c}
& {CPU} & {Mem.} & \multicolumn{2}{c|}{Network} &
\multicolumn{2}{c|}{Disk} \\\cline{4-7}
& & & Read & Write & Read & Write\\\hline
Bing DAGs & 0.76 & 1.01 & 1.69 & 7.08 & 1.39 & 1.94 \\\hline
Hive/ Hadoop & 0.89 & 0.42 & 0.77 & 1.34 & 1.59 & 1.41
\\\hlineHPC~(Condor) & 0.53 & 0.80 & N/A & N/A &
\multicolumn{2}{c|}{1.55 (R+W)} \\
\end{tabular}
}
\caption{Coefficient-of-variation~($={\mbox{stdev.}}/{\mbox{avg.}}$)
of tasks' demands for various resource. Across three examined
frameworks, tasks exhibit substantial variability~(CoV $\sim 1$) for many resources.\label{tab:resource_cov}}
\end{table}

\begin{table}
\centering
{\small
\begin{tabular}{p{.7in}|c|c|c|c|c}
\multirow{2}{*}{"Mass" that is \ldots}&
\multicolumn{5}{c}{Percentage of total work in the DAG}\\
& [0-20) & [20-40) & [40-60) & [60-80) & [80-100]\\\hline
{on CriticalPath} & 14.6\% & 13.2\% & 15.2\% & 15.3\% &
41.6\%\\%\hline
{"unconstrained"} & 15.6\% & 20.4\% & 14.2\% & 16.4\% &
33.3\%\\%\hline
{"unordered"} & 0 & 3.6\% & 11.8\% & 27.9\% & 56.6\% \\\hline
\end{tabular}
}\caption{Histogram of where the work in a DAG lies. For e.g.,
in $14.6\%$ of DAGs, the mass on their critical path is $\in [0,20)\%$ of the total work in that DAG.\label{tab:whereIsMass}}
\end{table}

Next, we were looking at how diverse are the resource demands?
Tasks in a stage have similar demands. Across nodes, however,
the demands vary. The more diverse the demands, the more need topack carefully.
%We find tasks have variable demands on four resources -- CPU
cycles, memory and the network and disk bandwidth that they needfor IO.
The variability is primarily due to the different work at each
node -- some are compute heavy~(e.g., user-defined code for
video rendering), others are memory heavy~(e.g., in memory
sorts) and still others are network heavy~(e.g., shuffles). The
coefficient-of-variation~(CoV) of the demands is shown in
Table~\ref{tab:resource_cov}. The CoV values indicate
substantial variability, hinting at the need to pack carefully.

\cut{
The relationship between variability in resource demands and thepotential for fragmentation
is not straightforward. We know, however, that the worst-case
performance ratio of a greedy packer increases linearly with thenumber of resources to be considered~\cite{}.
}

%How do the DAGs look? Figure~\ref{fig:snippets} illustrates
several stick figures; some DAGs are a chain of stages, others
are 'V's or 'W's where different chains end or start at a singlestage and still others have no discernible structure.

To understand the DAG structure better, we reason about where
most of the work lies.\robert{define work} We define CPMass as
the total work in stages that are on the critical path. By
UnconstrainedMass, we refer to the total work in stages that
have no parents. We also compute the maximal unordered mass
which is the work in the largest set of stages that are neither
parents nor children of each other. Table~\ref{tab:whereIsMass}
shows these results. We see that roughly 33\% of the DAGs have
unconstrained mass above 80\%. If the unconstrained mass
dominates, then ignoring dependencies cannot hurt too much sincemost work is in stages that are runnable. About 42\% of DAGs
have CPMass above 80\%; If CPMass dominates, then there is only
one chain of dependencies to cope with. The above cases are not
mutually exclusive and together account for 54\% of all DAGs.
The remaining 46\% of DAGs have mass distributed in a
substantially more complex manner. However, we also see that
57\% of DAGs have MaxUnorderedMass above 80\%. For these DAGs,
if parents of the unordered stages were scheduled appropriately,substantial gains can accrue from packing tightly the tasks in
this maximal unordered subset.

\cut{
Between dependencies and fragmentation, which is more important?We compute per DAG, the set of "unordered" tasks with the most
"work"; a pair of tasks are unordered if neither is an ancestor
nor a descendant of the other; we define work as
$\sum_{\mbox{task }t} \mbox{duration}_t * \mbox{demand}_{t,r}$
for bottleneck resource $r$. If a large fraction of the DAG's
work lies in the unordered subset, then packing this subset wellmay suffice to yield a good schedule. However, the largest
unordered set could lie somewhere in the middle of the DAG and apacker algorithm may be lead astray. So, as a conservative
estimate, we also compute per DAG the amount of work present in
its "unconstrained" tasks, i.e., tasks with no parents; these
tasks are immediately available for scheduling to the packer.
Table~\ref{tab:unconstr_masses} shows distributions of these
numbers. We find a wide range of DAG types. While some can be
scheduled well by just focusing on packability~(high fraction ofwork unconstrained or in unordered subsets), the vast majority
of DAGs require considering both dependencies and packing
together. {\bf SK: rephrase findings} Roughly half of DAGs have
substantial mass~(>80\%) on their critical path, so we have to
take care with dependencies. Roughly $40\%$ of DAGs have
substantial mass unconstrained, so simple packers will see some
benefit. However, if one were to be able to look at both, we seethat roughly $77\%$ of DAGs have some unordered subset with
substantial mass. {\bf sk: wtf}}

\begin{figure}
\includegraphics[width=1.5in]{figures/gap.pdf}
\caption{CDF of \emph{gap} between DAG runtime and several lowerbounds. Gap is computed as
$100\cdot\frac{runtime-lowerbound}{runtime}$.
\label{fig:gap}\fixme{redraw; squat; bigger font; better lines}}\end{figure}

To quantify the potential gains, we compare the runtime of the
DAGs in production at Bing with some lower estimates. The first
estimate is the duration of the DAG's critical path; a DAG wouldtake no longer if the available parallelism is infinite.
The second estimate is the total work in the DAG normalized by
the cluster share of that DAG.
If there were no dependencies and perfect packing, a DAG would
take no longer.
%Since all the work has to be done, a DAG would at least take solong and if there were no dependencies and no fragmentation, a
DAG would take exactly this long.
We define \emph{gap} as ${\small\sf
\frac{\mbox{duration}-\mbox{low estimate}}{\mbox{duration}}}$. Agap of 50\% implies 2$\times$ off the baseline. %and 75\% is
4$\times$ off.
Fig.~\ref{fig:gap} plots a CDF of these gaps over all the
observed DAGs.

The key observation is that half of the jobs have gaps of $70$\%and $86$\% w.r.t the above lower estimates. That is, half the
jobs take over $4\times$ longer than they should.
%Some DAGs are closer to their CPLength metric, others to their
TotalWork metric.
Note that these low estimates are loose-- the first ignores all
the work off the critical path and the second ignores
dependencies. We have developed a much tighter lower
estimate--BetterLB~(see~\xref{sec:betterlb}). The gap w.r.t
BetterLB decreases. However, half of the jobs are still off by
$45$\%.
We should mention a couple of caveats of our analysis. First,
some DAGs finish faster than their TotalWork metric. This is
because the production schedulers are work conserving and gives
more resources to jobs than their cluster share when spare
resources exist. Sedond, job runtimes are also impacted by
stragglers and failures~\cite{mantri}. The runtimes above
already discount these effects in two ways: (1) use the fastest
execution over groups of related jobs~(eg, recurring jobs
in~\cite{rope}) and (2) deduct the duration that the job spent
with $<10$ tasks executing.
We conclude that the runtimes in production are much better thanthe worst case analysis in~\xref{subsec:problem} but still
exhibit substantial room for improvement.


\cut{
The prevalence of each of the types of dependencies is as
follows.
A typical DAG has
$44.7\%$ of its inter-stage dependencies of the all-to-all
type,$34.1\%$ of its inter-stage dependencies of the many-to-one
type
and $21.2\%$ of its inter-stage dependencies of the one-to-one
type.
}

\subsection{Summary}
To summarize, we conclude with two observations. First,
production jobs have large DAGs with non-trivial structures thatare neither a bunch of unrelated stages nor a chain of stages.
Hence, scheduling these DAGs efficient requires respecting
dependencies and packing tasks across multiple resources and
time.
%Not doing so leads to {\em chokepoints} where too few tasks arerunnable and {\em fragmentation} where many resources are wastedbecause the runnable tasks won't fit within them.
Second, known algorithms fall into two main bins: they either donot handle diversity in resource demands (e.g., critical path
scheduling) and can be $O(n)$ off the optimal, or they do not
handle dependencies (e.g., Tetris) and can be $O(d)$ off the
optimal. Here, $n$ and $d$ are the numbers of nodes in the DAG
and resource dimensions respectively.

\cut{
So far, we have considered one DAG. But multiple jobs run
simultaneously in a cluster. We argue that the problems remain
similar but the solution complexity increases. Regarding the
problem, today's schedulers rely on fairness to pick a DAG,
i.e., whichever job is currently most under-allocated relative
to its desired share gets resources next~\cite{tetris}; then,
one of its runnable tasks is picked based on data locality.
Hence, the causes for {\em chokepoints} and {\em fragmentation}
carry over to the more general case. Regarding the solution, thecomplexity increases due to online job arrivals. Further, tasks
from many different jobs can run simultaneously on a machine, sopacking has to consider all active jobs and their runnable
tasks. Treating all of the jobs as a single DAG helps but is nota complete solution since (a) that cluster-wide DAG can be very
large leading to scalability issues during schedule computation
and more importantly (b) the completion time of the cluster-wideDAG relates to throughput (or makespan) but does not help reducethe completion time of individual DAGs or their average. Hence,
{\name} offers a different strategy to cope with multiple DAGs.
}


\cut{
\subsection{Model: Desired properties of a DAG scheduler}
{\bf edit: move to \S 3?}
Given a single DAG and a bounded resource capacity, a scheduler
should
finish execution in the shortest amount of time. Tasks have
demands
on resources and a duration, some of which are malleable, i.e.,
duration changes if fewer than peak resources are offered.
Also,task's demands can change with placement~(task placed on
same
machine
as input would not require network bandwidth).

Two challenges are new with multiple DAGs. One, is the
trade-offbetween speeding up a particular job versus speeding up
all jobs(makespan). Another, is the need to offer predictable
allocations
across groups of jobs (fixed guarantees are easy, but work
conserving
proportional fair allocations are harder). We are not aware of
any
prior work that considers dependencies and packing along with
these
aspects.
}


==> texfiles/old/ideas.tex <==
%!TEX root=../paper.tex
\section{Key ideas in {\namesec}}
\begin{figure}
\centering
\includegraphics[width=3in]{figures/arch.pdf}
\caption{{\name} in action\label{fig:arch}}
\end{figure}

In designing \name scheduler we focus on constructing a schedule for
DAG execution that approximates CP while minimizing cluster resource
fragmentation.   Specifically, since tasks can have different resource
requirements, the key ideas are to partition the DAG into {\em
  levels} (i.e., runnable vertices) which can then be packed tightly
based on cluster resource availability (see Figure~\ref{fig:arch}).



\subsection{Level scheduling}

Conceptually, we perform a topological sort of the DAG to construct
partitions of runnable vertices.  Our basic idea is to partition the
DAG into subsets such that (a) tasks in a subset have no dependencies
among themselves and (b) there exists a total order across subsets,
i.e., the subsets can be ranked numerically such that for every
dependency, the from-task is in a lower ranked subset than the
to-task.  An example is shown in Figure~\ref{fig:p_eg3}, where the
colored underlays represent the different subsets.

Our goal is to schedule the subsets in order produced by our
topological sort. That is, whenever a new resource becomes available
to the DAG, it is preferentially matched with tasks in subset order.
Matching does consider placement, i.e., tasks are preferentially
placed at machines where their resource use is small (e.g., data local
placements). The subsets are also carefully chosen to enhance
packability while respecting task dependencies. We use multi-resource
packing techniques to ensure that resources are not fragmented or
over-allocated (cf. Section~\ref{}).

An important aspect when scheduling per level order is the need to
adjust the schedule dynamically.  First, it is impossible to predict
precisely the durations of tasks; there could be runtime outliers or
failures.  Second, when many tasks remain in the most preferred
subset, it is likely that for every machine, some task exists in that
subset for which the machine is a good place. However, this may not
always hold. Especially when few tasks remain in the most-preferred
subset. Hence, rather than enforcing the subset order strictly, we
dynamically track dependencies and allow resources to be matched to
tasks in less preferred subsets as long as all (or a threshold
fraction) of their upstream tasks have finished.

Level scheduling has nice connections with widely-used algorithms; however the above version has a few novel aspects. Graph drawing tools~(e.g., GraphViz~\cite{XXX} and Microsoft AGL~\cite{XXX}) break a DAG into levels to enhance visiblity. So also do the early work on multi-processor scheduling; most notably the Graham-Coffman algorithm (G-C from now on)~\cite{XXX}. Even critical path scheduling can be thought of as a level scheduler~\footnote{Tasks' critical path length determines the level and the subset at each level consists of tasks having the same critical path length.}. We defer detailed comparisons to later~\xref{sec:related}, however none of the prior incarnations pick task subsets so as to enhance resource packability. Several do not consider placement constraints or allow for dynamic changes.

{\bf edit: perhaps good to directly pull out the clash with placement constraints. elevate main points.}

\subsection{Partitioning DAG into appropriate levels}
Input: a DAG of tasks. each task annotated with duration and resource use (vector over relevant dimensions).  We describe how to robustly estimate these task annotations from historical data (e.g., recurring jobs) and progress indications from tasks within the same stage.  Key: consider input size; placement.  And, an estimate of resource availability (this can change dynamically).

Output: partition of the DAG into levels as above; adjusts to track changes in resource availability.

Goal: Eventually, want good completion time of DAG. Sub-goal: pick subsets that are more packable together; larger subsets are better since they allow more leeway to match onto diverse offers; 
the degree of interruptions to critical path by levels should relate to the resources that are available; more resources => less interruption and vv; of course fewer interruptions imply limited scope to enhance packability.

\hrule

Algorithm: State = a DAG over task subsets. Initially, all the subsets are singletons. Recursively, merge the most {\em appropriate pair} of previously unordered subsets. Conclude when all subsets are strictly ordered. Appropriateness includes a few aspects; we pick based on a combined scoring function over the following parts. First, we measure how packable the subsets are; i.e., we measure the reduction in runtime between the case when the subsets execute individually (one after another) versus when they are scheduled together. We also call this the {\em compaction gain}.  Second, we measure the impact on the critical path due to a merger. Before the merger, some ancestors of the left subset could be scheduled before descendants of the right subset; but the merger prohibits this scheduling order. We measure this by comparing the critical path of the DAG before and after the merge; we call this the {\em CP inflation}.   Third, since we are greedily packing pairs of subsets, to get a proxy of global improvement we measure the total compaction gain of merge oppurtunities that are no longer allowed once a pair is merged. For example, ancestors of the left subset can no longer be merged with descendants of the right subset; so we count the potential compaction gains lost from all such pairs.  Greedily, we pick the subset that has the best combination score across these metrics.

To measure compaction gain, we emulate the dynamic scheduling algorithm described in~\xref{subsec:XXX} on the candidate subsets (individually and together). The emulation uses the number of available resources and hence, the subsets chosen crucially depends on the available resource amount.

At first blush, the above algorithm appears complex. However, through careful memoization, we show that it can be implemented within $O(n^2)$ calls to the emulation logic, where $n$ is the number of nodes in the DAG. In practice, we can run {\name} on a DAG of stages and $n$ is usually below $100$. The time to run an emulation is roughly linear in the number of nodes being emulated. So, the total runtime could be up to $O(2^n)$. However, we consider only subsets of tasks that are not ordered by the DAG, i.e., tasks that are neither ancestors nor descendants of each other; so the in practice, the runtime is much better.  For CP inflation, we compute the maximum distance from any root and to any leaf for each task; here root~(leaf) is defined as a task with no ancestors~(descendants).  When merging, we can compute these measures for the merged subset from the measures of the subsets being merged.  We do similar tricks to keep track of ancestors, descendants (for compaction gain lost) as well as to keep track of which subsets remain unordered.

{\bf edit: XXX, more things in the algorithm}
\hrule


\subsection{Multi-resource Packing}

We adapt a first-fit-decreasing heuristic for vector resources~\cite{vectorBinPack}.  Compared to prior work, we also consider task duration to be a resource dimension; not doing so leads to worse results especially when tasks can have very different durations (e.g., outliers or data skew).

\subsection{Packing: Over-allocation is useful, sometimes}
\label{subsec:overalloc}
Today's schedulers do not consider all the resources consumed by a task~(especially disk and network) during the assignment process which may lead to \textit{over-allocation} of these resources~\cite{tetris}. For example, if two tasks that can fully utilize the network are scheduled together, their completion time doubles.  Rampant over-allocation leads to poor performance since even though all of the resources appear utilized~(at 100\% usage for e.g.,) tasks are substantially delayed and collapse can happen~(e.g., too many seeks, memory thrashing, network incast).

Over-allocation is not always bad. When resources are constrained, it is often better to {\it slightly} over-allocate the fungible resources such as network and disk. Consider the following example: a scheduler which assigns tasks based on two resource demands: memory~(hard resource) and network~(fungible resource). Assume that each machine has the same capacity and each task requires 25\% memory and 40\% network~(percentages are over machine capacity).  Here, a machine can run two tasks at a time without over-allocation. If task duration is $1$, the per machine throughput is 2 tasks. However, if three tasks are scheduled simultaneously, network becomes over-allocated~(120\%) and the task duration increases to $1.2$. However, note that the per machine throughput is now $2.5$~($3 / 1.2$) tasks. Over-allocating further does not improve throughput. The key reason behind increase in throughput from slight over-allocation is that hard resources are being wasted otherwise due to fragmentation.

Over-allocation is not always useful. When other machines are free, it is better to schedule tasks on those machines rather than over-allocate. The reason is because over-allocation will increase task duration. 
%For example, consider two available machines and four tasks to schedule(same task profile as above), the cluster throughput is 4 units by spreading tasks. Over-allocating tasks on any machine is doing worse; allocating three tasks on a machine and one on the other machine leads to a total throughput of 3.33 units; assigning all four tasks to the same machine degrades it to 2.5 units. 
Similarly, if other tasks exist that can use the hard resources fully without over-fitting the fungible resources, it is often better to schedule them instead. 
%For example, given four tasks such as above, and four tasks that require 25\% memory and 0\% network, it is better to place two tasks that need network and two that do not, on each machine, for a machine throughput of 4 units. Placing any fewer tasks or running more tasks of the former or the latter type at any one time lowers the overall throughput. 

Packing schedulers such as Tetris never over-allocate. Production schedulers ignore network and disk. Hence, when cluster is busy, Tetris is inefficient. Whenever tasks have different usage profiles on network or disk, prior schedulers are inefficient. We show how to combine the best of both world when dealing with over-allocation. 

{\bf potential for gains in practice?}

\subsection{Fairness across DAGs}
\subsection{Average completion time vs. Makespan}

